Learning a Universal Template for Few-shot Dataset Generalization

Few-shot dataset generalization is a challenging variant of the well-studied few-shot classification problem where a diverse training set of several datasets is given, for the purpose of training an adaptable model that can then learn classes from new datasets using only a few examples. To this end, we propose to utilize the diverse training set to construct a universal template: a partial model that can define a wide array of dataset-specialized models, by plugging in appropriate components. For each new few-shot classification problem, our approach therefore only requires inferring a small number of parameters to insert into the universal template. We design a separate network that produces an initialization of those parameters for each given task, and we then fine-tune its proposed initialization via a few steps of gradient descent. Our approach is more parameter-efficient, scalable and adaptable compared to previous methods, and achieves the state-of-the-art on the challenging Meta-Dataset benchmark.

==> FLUTE (ICML 2021)/latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}

==> FLUTE (ICML 2021)/source/abstract.tex <==
\begin{abstract}
Few-shot dataset generalization is a challenging variant of the well-studied few-shot classification problem where a diverse training set of several datasets is given, for the purpose of training an adaptable model that can then learn classes from \emph{new datasets} using only a few examples. To this end, we propose to utilize the diverse training set to construct a \emph{universal template}: a partial model that can define a wide array of dataset-specialized models, by plugging in appropriate components.
For each new few-shot classification problem, our approach therefore only requires inferring a small number of parameters to insert into the universal template. We design a separate network that produces an initialization of those parameters for each given task, and we then fine-tune its proposed initialization via a few steps of gradient descent. Our approach is more parameter-efficient, scalable and adaptable compared to previous methods, and achieves the state-of-the-art on the challenging Meta-Dataset benchmark.
\end{abstract}
%For each new few-shot classification problem, learning the task therefore only requires inferring its `add-on' component. To this end, we design a separate network trained to produce a carefully-crafted initialization of the parameters of such `add-ons'. Our approach is more parameter-efficient, scalable and adaptable compared to previous methods, and achieves state-of-the-art on the challenging Meta-Dataset benchmark.

==> FLUTE (ICML 2021)/source/acknowledgements.tex <==
\section*{Acknowledgements}

\red{TODO: WRITEME.}

==> FLUTE (ICML 2021)/source/background.tex <==
\section{Background}
%We begin by defining the problem of few-shot classification and then introduce the more specific setup for the few-shot dataset generalization problem that is the focus of this work.
\paragraph{Few-shot Classification} Let $\mathcal{D}^{tr} = \{ (x_i, y_i) \}_{i=1}^{|\mathcal{D}^{tr}|}$ denote a (possibly large) training set, comprised of examples $x_i$ and their corresponding class labels $y_i$, with each $y_i \in  \mathcal{C}^{tr}$. That is, all of the training examples originate from a dedicated training set of classes $\mathcal{C}^{tr}$, while a disjoint validation set of classes $\mathcal{C}^{val}$ is also available for model selection. The aim is to use $\mathcal{D}^{tr}$ to obtain an \emph{adaptable} model that supports learning new classes from few examples.

Then, evaluation is carried out over a series of classification \emph{tasks}, or \emph{episodes}, designed to measure the trained model's ability to learn new classes from few examples. Specifically, a $k$-shot $N$-way test task presents $N$ classes from a set $\mathcal{C}^{test}$ that is disjoint from $\mathcal{C}^{tr}$ and $\mathcal{C}^{val}$. We denote each task as a tuple $\mathcal{T} = (\mathcal{S}_\mathcal{T}, \mathcal{Q}_\mathcal{T})$ of a `support set' and a `query set', representing small `within-task' training and test sets, respectively. The support set contains $k$ labeled examples of each of the $N$ classes: $\mathcal{S}_\mathcal{T} = \{ (x_1, y_1), \dots (x_{kN}, y_{kN}) \}$ with each $y_i \in \{ 1 \dots N \}$, while the query set $\mathcal{Q}_\mathcal{T} = \{ (x_1^*, y_1^*), \dots \}$ contains different (unlabeled) examples of the same $N$ classes.

Assuming a model with parameters $\theta$, the predicted label $\hat y^*$ of a query example $x^*$ is:
\begin{equation*}
    \hat y^* = \argmax_{y^* \in \{ 1 \dots N \}} \log p_{\theta}(y^* | x^*, \mathcal{S}_\mathcal{T})
\end{equation*}
% and therefore that model's average accuracy on task $\mathcal{T}$ is computed as:
% \begin{equation*}
%     \mathcal{A}_{\theta, \mathcal{T}} = \frac{1}{|\mathcal{Q}_\mathcal{T}|} \sum_{(x^*, y^*) \in \mathcal{Q}_\mathcal{T}} \mathbbm{1}[\hat y^* = y^*]
% \end{equation*}
% where $\mathbbm{1}[a = b]$ returns $1$ if $a = b$, else $0$
% Concretely, assuming $\theta$ denotes the model parameters, the model's prediction for a query example $x^*_u$ is:
% \begin{equation*}
%     \hat y^*_{u,t} = \argmax_{y^*_{u,t} = \{ 1 \dots N \}} \log p_{\theta}(y^*_{u,t} | x^*_{u,t}, \mathcal{S}_t)
% \end{equation*}
The evaluation metric is then the average query set accuracy over multiple few-shot classification tasks. 
%$\frac{1}{T}\sum_{\mathcal{T}} \mathcal{A}_{\theta, \mathcal{T}}$.

\paragraph{Few-shot Dataset Generalization} 
%\rz{I don't think we should switch to Domain, instead just stick to Dataset Generalization. Unless you have something else in mind here?}\et{oops yes, that was meant to say "dataset generalization" -- good catch Rich!} 
In this challenging instance of few-shot classification, the training and validation sets are defined as the union over $M$ different datasets:
\begin{align*}
    \mathcal{D}^{tr} &= \mathcal{D}^{tr}_1 \cup \mathcal{D}^{tr}_2 \dots \cup \mathcal{D}^{tr}_M \\
    \mathcal{D}^{val} &= \mathcal{D}^{val}_1 \cup \mathcal{D}^{val}_2 \dots \cup \mathcal{D}^{val}_M 
\end{align*}
where $\mathcal{D}^{tr}_m$ and $\mathcal{D}^{val}_m$ contain data from the dedicated training and validation sets of classes of dataset $m$, respectively. More compactly, we can view the training set (and analogously the validation set too) as $\mathcal{D}^{tr} = \{ (x_i, y_i, d_i) \}_{i=1}^{|\mathcal{D}^{tr}|}$, where the $x_i$'s and $y_i$'s denote examples and their corresponding class labels, as before, and $d_i$ denotes the dataset from which the associated example originates from.

Then, in keeping with the spirit of few-shot classification, the aim at evaluation time is to learn previously-unseen classes from few examples. However, in this more challenging setup, the new classes originate from \emph{new datasets} $\mathcal{D}_{M+1} \dots $, thus inducing a large generalization gap between the training set $\mathcal{D}^{train}$ and the test tasks. The evaluation metric now is the query set accuracy averaged over multiple tasks sampled from multiple held-out datasets.
% \begin{equation*}
%     \frac{1}{H} \sum_{h=1}^H \frac{1}{|\mathcal{T}_h|}\sum_{\mathcal{T}_h} \mathcal{A}_{\theta, \mathcal{T}_h}
% \end{equation*}
% where $\mathcal{T}_h$ denotes a few-shot task sampled from dataset $h$.

% \rz{Should have a background section on Film, and also earlier conditional formulations.}
\paragraph{Feature-wise Linear Modulation (FiLM)} FiLM \cite{dumoulin2018feature-wise} is a general-purpose conditioning mechanism that has been used extensively across diverse applications, like question answering, drawing a painting in the style of another, and so on. It performs an affine feature-wise transformation of its input $x$ based on a condition $d$:
\begin{equation*}
    \mathrm{FiLM}(x) = \gamma(d) \odot x + \beta(d).
\end{equation*}
The dependency of $\gamma$ and $\beta$ on $d$ is handled by maintaining distinct values for each setting of $d$ %(in our case we have $M$ different sets of $\gamma$'s and $\beta$'s, one per training dataset), 
and selecting the appropriate one for the forward pass of each example. 

==> FLUTE (ICML 2021)/source/conclusion.tex <==
\section{Conclusion}
To conclude, we proposed FLUTE, a method for few-shot dataset generalization that creates a universal template, i.e. a partially-parameterized model, that can serve to readily specify a good feature extractor for a held-out dataset, by simply plugging in an appropriate set of FiLM parameters. We propose an efficient approach for estimating those parameters, using a few steps of gradient descent starting from a task-dependent initialization. FLUTE sets the new state-of-the-art on Meta-Dataset, significantly outperforming previous methods on few-shot dataset generalization.

==> FLUTE (ICML 2021)/source/experimental_setup.tex <==
\section{Experimental Setup}
% \red{TODO: WRITEME.}

% \red{Experiments to consider:}
% \begin{itemize}
%     \item \red{How does our approach perform when using SUR-pf parameters? Do we also bridge the unseen domain performance gap? If our hypothesis holds, then SUR-pf --- which was trained on ImageNet-only first and which only trained the domain-specific parameters afterwards for the other training domains --- should {\em not} benefit from the inductive bias of training a set of shared parameters that lend themselves well to multiple sets of domain-specific parameters.}
    
%     \item \red{Visualization of the (multi-level) dataset classifier's outputs for different test episodes coming from seen and unseen domains.}
    
%     \item \red{Table that compares PEGASUS against approaches with the same number of parameters (CNAPs, Simple CNAPs, Meta-Baseline, TaskNorm, SUR-pf, URT-pf).}
    
%     \item \red{Table that compares PEGASUS against the state-of-the-art models (SUR and URT) that contain significantly more parameters.}
% \end{itemize}
We conduct our experimental evaluation on the recent Meta-Dataset benchmark, which lends itself well to studying few-shot dataset generalization, as its designated training set is indeed comprised of diverse datasets, and its test set includes classes from previously-unseen datasets too.

\paragraph{Meta-Dataset} In more detail, the training set contains classes from ImageNet, Omniglot, Aircraft, Birds, Flowers, Quickdraw, Fungi, and Textures, some of which contain natural images (e.g. ImageNet, Birds, and Flowers), while others differ significantly in appearance. For example, Omniglot and Quickdraw depict hand drawings on a plain black background and Textures's images present perceptual characteristics of varying structure and don't feature a single object in the center of the image. The test set introduces two new datasets: Traffic Signs and MSCOCO, with the former differing significantly thematically from the training set (it depicts images of different traffic signs), and the latter, albeit thematically similar to ImageNet, has lower resolution and exhibits inclusion. Since the aim of this work is to study few-shot dataset generalization, we incorporate the 3 additional test datasets introduced in \citet{requeima2019fast}, to obtain a larger and more varied test set for this problem. These datasets are MNIST, CIFAR-10, and CIFAR-100.

\paragraph{Strong versus weak generalization} The problem of few-shot dataset generalization requires \emph{strong generalization} as there is a large generalization gap between the training and test distributions. Another popular, albeit easier, setting creates the test tasks from held-out classes of the datasets that were encountered at training time. This still falls within the umbrella of few-shot classification, as the test classes were not used for training, but is an easier problem since the generalization gap is inherently smaller. We thus refer to this setting as \emph{weak generalization}. %it is more likely that a feature extractor that works well on the training classes of a particular dataset may also work well on the test classes of the same dataset. From that point of view, this setup is closer to the traditional single-dataset few-shot classification problem and presents a \empy{weak generalization} problem. 
Although our focus is few-shot dataset generalization in this work, we also examine FLUTE's performance on the weak generalization tasks for completeness and compatibility with previous work.

We apply FLUTE in exactly the same way for this setting as described in Section~\ref{sec:flute}. In particular, despite the test classes originating from seen datasets in this setting, we are not told which of the $M$ datasets each task is sampled from. %\rz{I like this point about not knowing the dataaet at test time. This could be highlighted more}.
Therefore, we still require our Blender network to propose a blending of the $M$ sets of FiLM parameters as the initialization of $\Psi_{d^*}$, although we expect that it should almost exclusively select the correct dataset from which the task originates, assuming the dataset classifier is accurate.

\paragraph{Implementation details} Following the prior work, we use a ResNet-18 as the feature extractor. During training of our universal template, we treat each dataset-specific readout head $r_m$ as a cosine classifier (as in \citet{chen2019closer, chen2020new}): a linear layer without a bias, where both the layer inputs and the rows of the weight matrix are l2-normalized. We use stochastic gradient descent with momentum as the optimizer for this phase, with a cosine decay with restarts schedule for the learning rate. On the other hand, the second phase of training for our dataset classifier network converges quite quickly (around 14K steps). The design of the dataset classifier involves a deep set encoder, comprised by 5 convolutional layers, each followed by batch normalization and ReLU, with a standard linear readout on top. We use Adam for this phase. We report all details in the Appendix and we will open-source our code upon publication.

==> FLUTE (ICML 2021)/source/experimental_setup_expanded.tex <==
\section{Experimental Setup}
% \red{TODO: WRITEME.}

% \red{Experiments to consider:}
% \begin{itemize}
%     \item \red{How does our approach perform when using SUR-pf parameters? Do we also bridge the unseen domain performance gap? If our hypothesis holds, then SUR-pf --- which was trained on ImageNet-only first and which only trained the domain-specific parameters afterwards for the other training domains --- should {\em not} benefit from the inductive bias of training a set of shared parameters that lend themselves well to multiple sets of domain-specific parameters.}
    
%     \item \red{Visualization of the (multi-level) dataset classifier's outputs for different test episodes coming from seen and unseen domains.}
    
%     \item \red{Table that compares PEGASUS against approaches with the same number of parameters (CNAPs, Simple CNAPs, Meta-Baseline, TaskNorm, SUR-pf, URT-pf).}
    
%     \item \red{Table that compares PEGASUS against the state-of-the-art models (SUR and URT) that contain significantly more parameters.}
% \end{itemize}
We conduct our experimental evaluation on the recent Meta-Dataset benchmark, which lends itself well to studying few-shot dataset generalization, as its designated training set is indeed comprised of diverse datasets, and its test set includes classes from previously-unseen datasets too.

\paragraph{Meta-Dataset} In more detail, the training set contains classes from ImageNet, Omniglot, Aircraft, Birds, Flowers, Quickdraw, Fungi, and Textures, some of which contain natural images (e.g. ImageNet, Birds, and Flowers), while others differ significantly in appearance. For example, Omniglot and Quickdraw depict hand drawings on a plain black background and Textures's images present perceptual characteristics of varying structure and don't feature a single object in the center of the image. The test set introduces two new datasets: Traffic Signs and MSCOCO, with the former differing significantly thematically from the training set (it depicts images of different traffic signs), and the latter, albeit thematically similar to ImageNet, has lower resolution and exhibits inclusion. Since the aim of this work is to study few-shot dataset generalization, we incorporate the 3 additional test datasets introduced in \citet{requeima2019fast}, to obtain a larger and more varied test set for this problem. These datasets are MNIST, CIFAR-10, and CIFAR-100.

\paragraph{Strong versus weak generalization} The problem of few-shot dataset generalization requires \emph{strong generalization} as there is a large generalization gap between the training and test distributions. Another popular, albeit easier, setting creates the test tasks from held-out classes of the datasets that were encountered at training time. This still falls within the umbrella of few-shot classification, as the test classes were not used for training, but is an easier problem since the generalization gap is inherently smaller. We thus refer to this setting as \emph{weak generalization}. %it is more likely that a feature extractor that works well on the training classes of a particular dataset may also work well on the test classes of the same dataset. From that point of view, this setup is closer to the traditional single-dataset few-shot classification problem and presents a \empy{weak generalization} problem. 
Although our focus is few-shot dataset generalization in this work, we also examine FLUTE's performance on the weak generalization tasks for completeness and compatibility with previous work.

We apply FLUTE in exactly the same way for this setting as described in Section~\ref{sec:flute}. In particular, despite the test classes originating from seen datasets in this setting, we are not told which of the $M$ datasets each task is sampled from. %\rz{I like this point about not knowing the dataaet at test time. This could be highlighted more}.
Therefore, we still require our Blender network to propose a blending of the $M$ sets of FiLM parameters as the initialization of $\Psi_{d^*}$, although we expect that it should almost exclusively select the correct dataset from which the task originates, assuming the dataset classifier is accurate.

\paragraph{Implementation details} Following the prior work, we use a ResNet-18 as the feature extractor. During training of our universal template, we treat each dataset-specific readout head $r_m$ as a cosine classifier (as in \citet{chen2019closer, chen2020new}): a linear layer without a bias, where both the layer inputs and the rows of the weight matrix are l2-normalized. We use stochastic gradient descent with momentum as the optimizer for this phase, with a cosine decay with restarts schedule for the learning rate. On the other hand, the second phase of training for our dataset classifier network converges quite quickly (around 14K steps). The design of the dataset classifier involves a deep set encoder, comprised by 5 convolutional layers, each followed by batch normalization and ReLU, with a standard linear readout on top. We use Adam for this phase. We report all details in the Appendix. Our code is publicly available and has been incorporated into the Meta-Dataset codebase\footnote{https://github.com/google-research/meta-dataset}.

==> FLUTE (ICML 2021)/source/introduction.tex <==
\section{Introduction}
While deep learning approaches have recently driven remarkable progress on many important applications, their ability to rapidly learn new concepts from small datasets is significantly lacking. This observation has inspired research towards creating more flexible and adaptable methods. A well-studied problem in this direction is few-shot classification: the problem of utilizing a (possibly large) labeled training set to create an \textit{adaptable} model that is then capable of learning new classes from few examples. Concretely, a few-shot learning model is evaluated on test {\em tasks}, each of which poses a classification problem between previously-unseen classes, given only a few examples of each. %Within each episode, the model is given a few labeled examples (the `support set') to learn about the new classes, and is then asked to classify a disjoint subset of unlabeled examples of those new classes (the `query set').

% Early benchmarks for this problem like Omniglot and \textit{mini}-ImageNet, divide a particular dataset's classes into disjoint sets: one that can be used for training, and another that is used to create the test-time classification tasks. Due to this construction, the classes seen at training and evaluation times are related, e.g. they have similar appearance and likely depict similar concepts, due to having originated from the same dataset. This allows to obtain strong performance on these benchmarks by largely re-using features learned on the training set when asked to solve each test-time task.

% Despite the initial popularity of those benchmarks, they unfortunately are a poor proxy for real-world scenarios, since in practice we typically don't have a homogeneous training set all of which is relevant for the downstream task(s) of interest. This has inspired recent work \cite{triantafillou2020meta,requeima2019fast,bateni2019improved,bronskill2020tasknorm,saikia2020optimized,dvornik2020selecting,liu2020universal} to pivot towards a more realistic and challenging variant of few-shot classification where the training set is comprised of classes originating from multiple diverse datasets, or `domains'. At evaluation time, two types of few-shot classification tasks are considered: ones that are formed from held-out classes of the domains encountered during training, and others that are formed from classes originating from entirely-unseen domains (`out-of-domain episodes'). The latter category is significantly more challenging than the former, due to its inherent larger generalization gap from the training set. However, we argue that making progress on the out-of-domain tasks will have the largest real-world impact, and this is the focus of our work.

Departing from early benchmarks for this problem, recent work is shifting towards a more challenging instance of few-shot classification \emph{across datasets} \cite{chen2019closer,tseng2020cross,triantafillou2020meta,requeima2019fast,bateni2019improved,bronskill2020tasknorm,saikia2020optimized,dvornik2020selecting,liu2020universal}. Similarly, we consider the challenging problem of \textit{few-shot dataset generalization}, where the training set is comprised of classes originating from multiple diverse datasets, like ImageNet, Omniglot, Aircraft, and so on, and the aim is to utilize this diverse data towards building a model that can solve new classification tasks between classes of previously-unseen datasets at test time, using only a few examples.
%The aim then, at evaluation time, is to solve two types of few-shot classification classification tasks: ones that are formed from held-out classes of the datasets encountered during training, and others that are formed from classes originating from entirely-unseen datasets (`out-of-domain episodes'). The latter category is significantly more challenging than the former, due to its inherent larger generalization gap from the training set. However, we argue that making progress on the out-of-domain tasks will have the largest real-world impact, and this is the focus of our work.

Few-shot dataset generalization exhibits the same challenge of data scarcity as its traditional (single-dataset) few-shot classification counterpart, but it also presents two additional difficulties. Firstly, the heterogeneous nature of the training dataset is reminiscent of \emph{multi-task learning}~\citep{caruana1997multitask}, 
%\rz{should include citations here and for dom gen below}
where care must be taken to avoid interference when training jointly for different objectives, or different datasets in this case. 
%\rz{Not clear how compactness relates to dataset interference. Should this be a 3rd issue, of scalability?}\et{I actually removed that sentence because I agree it seemed odd there, and we're later expanding on our scalability and parameter compactness anyway, so I didn't think it added much here.}
Secondly, the fact that the test-time tasks are composed of classes from previously-unseen datasets breaks the i.i.d. assumption, resembling the problem of \emph{domain generalization} \cite{gulrajani2020search}. In a nutshell then, to succeed in few-shot dataset generalization, a method must 1) ingest diverse information without interference, and 2) define a mechanism to appropriately re-purpose that acquired knowledge in order to accommodate extensively different data at test time, using few examples. %We aim to address this challenge without sacrificing compactness, by ensuring that our model's number of parameters scales well with the number of training datasets.

In this work, we propose to tackle this problem by learning a {\em universal template}: a partially-parameterized model trained on multiple datasets in parallel that can be used to define a wide array of dataset-specialized models by providing values for the remaining parameters. We posit that this design incorporates a useful inductive bias for few-shot dataset generalization: in addition to benefiting from knowledge acquired on diverse data, it also reflects the requirement that the template should be flexible enough to serve as the basis to parameterize a diverse set of task-solving networks. %The intended effect of this inductive bias is to provide the flexibility to adapt to very different tasks in an efficient manner, which is critical in the data-scarce regime we study.%\rz{Parameter-light is an odd term. Maybe just efficient?}

% We propose to use conditional batch normalization~\cite{de2017modulating} --- a form of feature-wise transformation~\cite{dumoulin2018feature-wise} --- as a concrete instantiation of this framework. In this case the shared template consists of the convolutional kernels of a residual network~\citep{he2016deep} and the task-specific parameters to be filled-in are the batch normalization layers' scaling and shifting coefficients.
%We train the architecture jointly across diverse training datasets using FiLM~\citep{perez2018film} for task specialization via conditional batch normalization. 
To this end, we propose to train a feature extractor jointly across diverse datasets using FiLM~\citep{perez2018film} in the form of conditional batch normalization: we share the parameters of the convolutional layers across datasets, but allocate a separate set of batch normalization parameters for each.
This joint training regime is key for creating a universal template: by forcing the batch normalization parameters to be fully responsible for dataset specialization, our training objective ensures that the convolutional parameters are \emph{general}, and thus indeed act as a universal template that is able to support generalization to vastly different datasets. To then tackle test-time tasks from unseen datasets, we propose to use the few available labeled examples of each given task to \emph{learn} a new set of batch normalization parameters for that task, starting from a task-dependent initialization: a combination of the per-dataset trained sets of parameters whose co-efficients are proposed by a separate learned network. We refer to this as Few-shot Learning with a Universal TEmplate (FLUTE), illustrated in~\autoref{fig:flute_diagram}.
% vdumoulin, etriantafillou: done.
% \rz{Is there space for a model figure?}

% Concretely, we instantiate this framework in the context of a residual network, where the shared template is given by the convolutional weights, and dataset specialization is achieved via different settings of the batch normalization layers. We train this architecture jointly across all training datasets using Feature-wise Linear Modulation (FiLM) \cite{dumoulin2018feature-wise} in the form of conditional batch normalization, to distinguish the forward passes of data belonging to different datasets. This joint training regime is key for creating a universal template: by forcing the batch normalization parameters to be fully responsible for dataset specialization, our training objective ensures that the convolutional parameters are \emph{general}, and thus indeed act as a universal template that is able to support generalization to vastly different datasets. To then tackle test-time tasks from unseen datasets, we propose to use the few available labeled examples of each given task to \emph{learn} a new set of batch normalization parameters for that task, starting from a carefully-constructed initialization: a convex combination of the per-dataset trained sets of batch normalization parameters, where the combination co-efficients are proposed by a separate learned network. We refer to this approach as Few-shot Learning with a Universal TEmplate (FLUTE).

We experimentally evaluate FLUTE on few-shot dataset generalization using the recent Meta-Dataset benchmark \cite{triantafillou2020meta} that is comprised of 10 diverse datasets, 8 of which can be used for training, with the remaining 2 reserved for evaluation. To obtain a richer set of evaluation tasks, we incorporate 3 additional evaluation-only datasets, following \citet{requeima2019fast}. FLUTE significantly outperforms the state-of-the-art on few-shot dataset generalization on Meta-Dataset (by $>$ 5\%), despite having significantly fewer parameters (approx. 8 times fewer).

Aside from its strong performance, FLUTE has several advantages over previous approaches. Firstly, it is more scalable: it's more parameter efficient, produces more parsimonious representations, and has favorable test-time computational complexity, as summarized in Table~\ref{table:flute_vs_sur_urt}. It is also very expressive since, for each test task, it blends the per-dataset trained parameters in \emph{all} representation levels (in the batch normalization layers throughout the network), and it is easily adaptable due to its efficient training of a small subset of the feature extractor's parameters in each test task.
% \begin{itemize}
%     \item {\em Parameter efficiency}: its number of parameters scales well with the number of training datasets.
%     \item {\em Parsimony}: the size of the representations it produces does not grow with the number of training datasets.
%     \item {\em Computational efficiency}: the number of forward and backwards passes required in each few-shot classification task does not grow with the number of training datasets.
%     \item {\em Expressivity}: for each task, it blends the per-dataset trained parameters in \emph{all} representation levels (in the batch normalization layers throughout the network), instead of only in the top-most embedding space.
%     \item {\em Adaptability}: it trains a new set of batch normalization parameters for each task. This is crucial for addressing vastly different data at test time.
% \end{itemize}
% In what follows, we formally define the problem of few-shot dataset generalization; then we introduce FLUTE; we discuss related work; present our extensive experimental evaluation; and finally we conclude by discussing open directions for future work.
% \rz{can omit outline if we need space}

%Architecturally, this design is identical to the parametric families of SUR and URT, but our model is trained for a different purpose. Aside from parameter-efficiency, we argue for the use of a parametric family model as an inductive bias in and of itself: we posit that a universal skeleton that can be readily completed with task-specific `add-ons' constitutes an effective vehicle for appropriately leveraging previously-acquired diverse knowledge, while at the same time allowing the flexibility to adapt to vastly different tasks. Our model learns a new set of batch normalization parameters for each given task at evaluation time, starting from a carefully-constructed initialization via a convex combination of the trained per-dataset batch normalization parameters whose weights are proposed by a learned network. %Despite its simplicity and parameter efficiency, our model achieves state-of-the-art on the challenging Meta-Dataset benchmark, outperforming even SUR and URT that have significantly more parameters.

%Recently, significant progress was made in this direction by SUR \cite{dvornik2020selecting} and URT \cite{liu2020universal} that construct `universal representations': a term coined in \cite{bilen2017universal} to describe a rich set of features that enables strong performance on multiple datasets. To tackle each evaluation task then, a selection mechanism is employed that identifies a subset of the universal representation that is relevant for the task at hand, and subsequently a simple nearest-centroid algorithm is applied on top of the selected features to perform the given classification task. Because these approaches train a separate feature extractor for each training source, they side-step any potential interference issues, but fail to meet our desideratum of parameter-efficiency. To mitigate this, SUR and URT also offer `parametric family' variants, SUR-pf and URT-pf, respectively, where the per-dataset feature extractors share all but their batch normalization parameters. Unfortunately, though, the compactness of their parametric family models comes at the cost of a significant accuracy drop on most downstream few-shot classification tasks.

%In this work, we advocate for a different notion: building a `universal \emph{skeleton}': a network that serves as a \emph{template} for defining a wide array of task-specialized models, each of which is obtained by `plugging in' a different set of batch normalization parameters. Architecturally, this design is identical to the parametric families of SUR and URT, but our model is trained for a different purpose. Aside from parameter-efficiency, we argue for the use of a parametric family model as an inductive bias in and of itself: we posit that a universal skeleton that can be readily completed with task-specific `add-ons' constitutes an effective vehicle for appropriately leveraging previously-acquired diverse knowledge, while at the same time allowing the flexibility to adapt to vastly different tasks. Our model learns a new set of batch normalization parameters for each given task at evaluation time, starting from a carefully-constructed initialization via a convex combination of the trained per-dataset batch normalization parameters whose weights are proposed by a learned network. %Despite its simplicity and parameter efficiency, our model achieves state-of-the-art on the challenging Meta-Dataset benchmark, outperforming even SUR and URT that have significantly more parameters.

% We refer to our approach as Parameter-Efficient Generalization Across Sources with a Universal Skeleton (PEGASUS). It has several advantages:
% \begin{itemize}
%     % \item Parameter-efficiency: like SUR-pf and URT-pf, but unlike SUR and URT, our number of parameters does not grow with the number of training sources.
%     \item Parameter-efficiency and compactness: our number of parameters does not grow with the number of training datasets, and neither does the size of our representations, contrary to previous work.
%     % \item Favourable computational complexity, especially if the number $N$ of training sources is large: Each of SUR(-pf) and URT(-pf) requires $2N$ feature extractor forward passes for each task. In contrast, we only require $2T + 1$ forward and backward passes, where $T$ is the number of steps for training the batch normalization parameters for the task which in practice is small.
%     % \item Compactness of representations: While SUR(-pf) produces representations whose size grows with the number of training sources, the size of our representations is constant.
%     \item Expressivity: For each new task, we `blend' the trained per-dataset backbones on {\em all} levels of representation (by learning batch normalization parameters for all layers of the network). %In contrast, SUR(-pf) and URT(-pf) only combine the trained backbones on the top-most level.
%     \item Adaptability: Our inductive bias of a shared skeleton, paired with our mechanism for adaptation constitutes a very adaptable approach, allowing to significantly outperform previous work on out-of-domain episodes. %In fact, we significantly outperform even SUR and URT which have significantly more parameters on several out-of-domain tasks.
%     \item Strong performance: Overall, our approach sets a new state-of-the-art on the recent Meta-Dataset benchmark \cite{triantafillou2020meta}, surpassing the performance of even significantly parameter-heavier approaches.
% \end{itemize}


% % \red{TODO: WRITEME.}

% \red{vdumoulin's proposed story line: SUR~\citep{dvornik2020selecting} shows that the multi-domain representation obtained by weighting and concatenating domain-specific representations is a good representation for few-shot classification, and its parametric family variant is a parameter-efficient way of defining the domain-specific representations. In this work, we explore the use of parametric families of networks to represent domain-specific models as an inductive bias in and of itself: rather than forming a multi-domain representation, we posit that the shared parameters lend themselves well to learning a new set of domain-specific parameters on a new classification episode, and a combination of the domain-specific parameters learned during training is a good initialization for those parameters.}

% \red{This approach provides several advantages:}

% \red{\begin{itemize}
%     \item Its increased adaptability allows the model to perform better on out-of-domain episodes.
%     \item For large parametric families (very large number N of training domains), its computational complexity is more advantageous: while SUR requires $2N$ forward passes through the domain backbones, our approach requires $2T + 1$ forward and backward passes, where $T$ is the number of fine-tuning steps.
%     \item The resulting representation has a constant size with respect to the size of the parametric family.
%     \item Rather than combining representations from top-most embeddings, like SUR or URT, our approach blends the trained backbones' parameterizations at {\em all} abstraction levels. (vdumoulin: I don't know if it's very clear for a casual reader, maybe we should elaborate?)
% \end{itemize}}

% \red{Suggestion by Rich: sell our strong generalization results. Eleni: for weak generalization, we do almost as well as 8-backbone models, which have a lot more parameters.}


==> FLUTE (ICML 2021)/source/model.tex <==
\section{Introducing FLUTE}\label{sec:flute}

\begin{figure*}[t]%
    \centering%
    \includegraphics[width=0.48\linewidth]{figures/flute_diagram.pdf}%
    \hfill%
    \includegraphics[width=0.48\linewidth]{figures/flute_diagram_blender.pdf}%
    \caption{\label{fig:flute_diagram}({\em Left}) FLUTE trains the shared convolutional weights comprising the universal template, and the $M$ dataset-specific sets of FiLM parameters ($M = 2$ in this illustration) using a multi-task classification loss. ({\em Right}) The FiLM parameter values for a test episode are learned through gradient descent using a nearest-centroid classifier (NCC) fitted on the support set as the output layer. The {\em Blender network} is used to initialize the new FiLM parameters as a convex combination of the trained sets of FiLM parameters. %\rz{Should mention tuning step after initialization.} %the FiLM parameter initialization: it outputs  a convex combination of the training datasets' FiLM parameters, with the combination coefficients corresponding to the probabilities output by a training dataset classifier.}%
    }
\end{figure*}

At a high-level, the core idea behind FLUTE is to use multiple diverse training datasets to construct a \emph{universal template} that can represent a wide array of dataset-specific feature extractors by filling in the shared template with appropriate parameters. % by providing values for the task-specific parameters. 
During training, FLUTE learns $M$ such sets of dataset-specific parameters, one per dataset in $\mathcal{D}^{train}$. 

We propose to use FiLM on batch normalization layers (also known as conditional batch normalization~\citep{de2017modulating}) as a concrete instantiation of this framework. The shared template therefore consists of the convolutional kernels of a residual network~\citep{he2016deep}, and the dataset-specific parameters to be filled-in are the batch normalization layers' scaling and shifting coefficients, which we refer to as the \emph{FiLM parameters} from now on. %In other words, the dataset-specific components that we plug into the universal template take the form of different sets of batch normalization parameters, which we refer to as {\em FiLM parameters} from now on.

% Specifically, we choose FiLM as the means of specializing the universal template to tasks of different datasets, where the condition is the dataset identifier. As is often the case in practice, instead of inserting additional FiLM layers in the network's architecture, we modulate the scaling and shifting parameter values of existing batch normalization layers~\citep{dumoulin2017learned,de2017modulating}. In other words, the per-dataset components that we plug into the universal template take the form of different sets of batch normalization parameters, which we refer to as FiLM parameters from now on.

Our reason for choosing FiLM for this purpose is two-fold. First, while simple, it is very expressive and flexible, as evidenced by its wide success in vastly different problem settings~\citep{dumoulin2018feature-wise}. This is very important for our goal of generalizing to extensively different data. Second, FiLM layers contain a small fraction of a network's overall parameters, which is crucial for our few-shot setting where limited data is available for learning how to specialize our template to test tasks of different datasets.

At evaluation time, for each test task, our goal is to produce a new set of FiLM parameters that yields a good feature extractor for that task when plugged into the universal template. We propose to \emph{learn} such parameters through gradient descent on the given task's support set. In doing so, we also need to specify how to initialize the new FiLM parameters. In practice, we find that initialization really matters, and that simply performing more gradient steps is insufficient to recover from a bad initialization. We propose a simple heuristic that we find works well in practice: initialize a new task's FiLM parameters from a convex combination of the training datasets' FiLM parameters where the combination weights are a function of how ``compatible'' each training dataset is with the new task. We define this ``compatibility'' to be the output of a dataset classifier that discriminates between the $M$ training datasets. We refer to this approach in what follows using the term \emph{Blender network}.

In what follows, we first describe how we train our universal template, FiLM parameters, and Blender network, and then present our algorithm for tackling few-shot classification tasks from previously-unseen datasets.%\rz{I don't know that we have sufficiently motivated why it is useful to have separate batch norm params per dataset - is there some reason why these are the right parameters to adapt in the template?}\et{Good point! I added a paragraph in this section to address this - let me know what you think.}

\subsection{Training the universal and per-dataset parameters} 
%Like SUR-pf and URT-pf, we define a \emph{parametric family} of per-dataset feature extractors that share all but their batch normalization parameters. To achieve this, SUR-pf and URT-pf train their feature extractors sequentially, by first training a feature-extractor on ImageNet only, and then freezing the shared weights and only allowing each of the remaining datasets to learn a dedicated set of batch normalization parameters, without modifying the shared weights. In contrast, we train the shared weights on data from \emph{all} training domains, during a single joint training phase.
%This design choice of allowing all training datasets to influence the shared weights is crucial for the goal of creating a \textit{universal skeleton} that supports strong performance on multiple sources: it encourages the shared weights to be as general as possible, and thus more apt to accommodate a wide-range or diverse tasks via a parameter-light task specialization through batch normalization parameters.
We define our universal template as the convolutional layer parameters of our ResNet-18 feature extractor, and the dataset-specific components take the form of FiLM parameters via different settings for the batch normalization layers.

%We train our feature extractor jointly over all $M$ training datasets and utilize a conditioning mechanism to distinguish the processing of examples coming from different datasets. In particular, we use Feature-wise Linear Modulation (FiLM) \cite{dumoulin2018feature-wise}, in the form of conditional batch normalization. Specifically, let $\gamma^i$ and $\beta^i$ denote the batch normalization parameters for layer $i$, for scaling and shifting, respectively. While in a standard batch normalization layer the size of each of $\gamma^i$ and $\beta^i$ is the number $c^i$ of channels in layer $i$, in our case $\gamma^i$ and $\beta^i$ have shape $[M, c^i]$. In other words, there is a separate set of batch normalization parameters \emph{per training dataset}. %To forward pass a training example through our feature extractor, then, we utilize the scaling and shifting parameters dedicated to the dataset from which that example came from, throughout the forward-pass, by selecting exactly one row of each of $\gamma^i$ and $\beta^i$. We will later discuss how we perform the forward pass through these layers when the source is unknown at test time. %At test time, when the source is unknown, we devise a mechanism for selecting from the sets of batch normalization parameters in a soft way, using our combiner network that we discuss later.

We train our feature extractor \emph{jointly} over all $M$ training datasets, and we maintain $M$ sets of FiLM parameters for distinguishing the forward passes of examples of different datasets. Formally, let $f$ denote our feature extractor function, and let $\Phi$ and $\Psi$ be the shared universal template parameters (the convolutional layer parameters of $f$) and the dataset-specific  parameters, respectively, with $\Psi_m$ (row vector of $\Psi$) denoting the FiLM parameters for dataset $m$. Finally, let $\Omega$ denote the parameters of per-dataset classification readout heads $r_1, \dots r_M$, where the readout layer $r_m$ for dataset $m$ has $|\mathcal{C}^{tr}_m|$ units and is parameterized by $\Omega_m$.

Then, each update to the model is computed as follows: we sample a batch $\mathcal{B}$ of data from the training set $\mathcal{B} = \{ (x_i, y_i, d_i) \}_{i=1}^{|\mathcal{B}|}$, with each element $i$ of the batch being a tuple that contains an image $x_i$, its one-hot-encoded class label $y_i$, and its one-hot encoded dataset label $d_i$. We compute the network's prediction of the class label $\hat y_i$ as follows:
\begin{equation*}
    \hat y_i = r_{d_i}(f(x_i; \Phi, \Psi_{d_i}); \Omega_{d_i})
\end{equation*}
We then train $\Phi$, $\Psi$, and $\Omega$ to minimize the cross-entropy loss:
\begin{equation*}
    - \sum_{i=1}^{|\mathcal{B}|} y_i \log \hat y_i 
\end{equation*}

Notice that the loss of an example $x_i$ influences only the FiLM parameters corresponding to its originating dataset $d_i$, but \emph{all} examples influence the shared parameters $\Phi$. We posit that this design is essential for rendering $\Phi$ a \emph{universal} template that is general enough to enable dataset specialization to a wide range of diverse datasets by merely changing the values of the parameter-light batch normalization layers.

After this phase, we no longer require the per-dataset  readout heads $r_1, \dots r_M$, so we discard them at this point.

\subsection{Training the Blender network}
The purpose of this network is to create (an initialization for) the FiLM parameters for an unseen dataset $d^*$ via appropriately blending the $M$ sets of FiLM parameters $\{ \Psi_m \}_{m=1}^M$. The aim, in particular, is to yield a good feature extractor for $d^*$ by in-filling the universal template with these new FiLM parameters. We define the blending operation as a convex combination whose co-efficient for a particular dataset $m$ is given by an estimate of compatibility between $m$ and $d^*$.

%Recall that the ultimate aim of FLUTE is to tackle few-shot classification tasks of new datasets. %In fact, in the particularly interesting and important case of out-of-domain tasks, the episodes at test time come from previously unseen sources for which we do not even possess per-dataset parameters. The challenge is thus to come up with a set of batch normalization parameters for each test episode that, when inserted into the shared universal template, yield a good feature extractor for solving that episode's classification task. Towards this goal, we aim to \emph{learn} a new set of batch normalization parameters for each test episode using its support set, as described in the following sub-section. We now discuss how to construct the initialization for that learning phase.

%Intuitively, if a test task is sampled from a dataset that largely resembles a particular training dataset $m$, then $\Psi_m$ may be a good choice for the batch normalization parameters for this new task. To leverage this intuition, we therefore require an estimate of the compatibility between a given test task and each of the trained per-dataset parameters.
Towards estimating that compatibility, we propose to train a \emph{dataset classifier}: a network that reads a batch of data and predicts which of the training datasets it was sampled from. The idea is then to interpret this dataset classifier's probablities as a proxy for the compatibility between the data it ingested and each training dataset.

Formally, let $g$ denote a network that takes as input a \emph{set} of examples $\mathcal{B}$ and creates a vector representation of that set. We use a permutation-invariant `set encoder' \cite{zaheer2017deep} for $g$ that we describe in the Appendix. Also let $l$ denote a $M$-dimensional linear readout layer. %We train this network to read a set of examples of the same dataset, create a set representation of it, and use that to predict the dataset from which the batch of examples originated. This utility of this design choice lies in the ability to ingest a `support set' at test time and produce the probabilities that it belongs to each training dataset.

Each update to the parameters of $g$ and $l$ is performed by first sampling a training dataset $m$ (an integer between $1$ and $M$), and then sampling $\mathcal{B}$ from $\mathcal{D}^{tr}_m$. We compute the dataset classifier's logits as $\hat d = l(g(\mathcal{B}))$, and we train the parameters of $g$ and $l$ to minimize the cross-entropy loss for the dataset classification problem. %Let $d = \onehot(m)$ denote the one-hot encoded dataset label and $\hat d$ the dataset classifier's probabilities: $\hat d = \softmax(r(g(\mathcal{B})))$. We train the parameters of $g$ and $r$ to minimize the cross-entropy loss $- d \log \hat d$ for the dataset classification task.

Once the dataset classifier is trained, we define the blender function as
\begin{equation*}
    \blend(\mathcal{B}) = \softmax(l(g(\mathcal{B})))^T\Psi
\end{equation*}
In words, this is a convex combination of the trained sets of FiLM parameters (the rows of $\Psi$), where the combination co-efficients are the probabilities of the given batch of data $\mathcal{B}$ of unknown origin belonging to each of the training datasets.
%Intuitively, for an episode that is sampled from (held-out classes of) one of the training sources $d$, a good candidate for the batch normalization parameters to use is $\Psi_d$. In this case, therefore, we require a way to predict which of the training sources the given episode comes from, as that information isn't given at test time. On the other hand, when given an out-of-domain episode, perhaps the best choice is to use the parameter $\Psi_d$ of the dataset $d$ that is the most \emph{compatible} with the support set of the given episode. We hypothesize that we can tackle both of these cases via learning a \emph{dataset classifier}: a network that ingests a batch of data coming from a particular training source and aims to predict that source. We then directly treat the probabilities of this dataset classifier as the weights with which to blend the batch normalization parameters of each of the training sources in order to create a set of batch normalization parameters for the newly encountered data.

% In its simplest form, our architecture consists of a 5-layer convolutional neural network, followed by global average pooling, and averaging over the batch dimension, in order to obtain a “deep set encoding” of the given batch of data. We add a readout layer on top of that deep set representation for the dataset classification task, and we train these new components using the cross-entropy loss. 

% Building on this idea further, we hypothesize that it would be beneficial to learn more than one “classification heads”, at different levels of representation. This is a more modular design, as a particular unseen dataset might not be too similar to any of the seen ones overall, but it still might bear similarity to certain seen datasets on certain levels of representation. For example, the optimal FiLM parameters for each of Omniglot and Quickdraw might be similar to each other in low representation levels (since both of these datasets involve simple drawings with a black background) but more distinct in higher levels (since the concepts depicted in each of those datasets are different). To achieve this, we insert a linear readout layer for dataset classification after each of the 5 layers in the convolutional neural network that is being trained in this phase. The training objective is now the cross-entropy for the dataset classification task, averaged over the 5 different sets of dataset classification logits.

\subsection{Tackling few-shot test tasks}
Let $\mathcal{T} = \{ \mathcal{S}_{\mathcal{T}}, \mathcal{Q}_{\mathcal{T}} \}$ denote a few-shot test task coming from an unseen dataset $d^*$. Our approach to solving $\mathcal{T}$ can be broken down into two steps. First, we define a feature extractor for $\mathcal{T}$ via an appropriate in-filling of the universal template, and second, we predict a class label for each query example via a simple algorithm that operates on top of the constructed feature extractor.

\paragraph{Step 1: Defining the feature extractor} In this step, we seek a set of FiLM parameters $\Psi_{d^*}$ for the given task of unseen dataset $d^*$ that yield a good feature extractor $f(\cdot ; \Phi, \Psi_{d^*})$ when plugged into the universal template.

We initialize $\Psi_{d^*}$ to the convex combination proposed by the blender network based on the task's support set:
\begin{equation*}
    \Psi_{d^*}^{init} = \blend(\mathcal{S}_{\mathcal{T}})
\end{equation*}

Then, we use gradient descent to train $\Psi_{d^*}$ from the initialization $\Psi_{d^*}^{init}$. We next describe the training objective that we use for that purpose, using a Nearest-Centroid Classifier.

\paragraph{Nearest-Centroid Classifier (NCC)}
%Given a task $\mathcal{T} = \{ \mathcal{S}_{\mathcal{T}}, \mathcal{Q}_{\mathcal{T}} \}$, a model must classify each query set example into one of the newly-presented $N$ classes after having used the support set to learn about those classes. NCC is a simple but effective method for achieving this \cite{snell2017prototypical,chen2019closer,chen2020new}.
The NCC \cite{mensink2013distance,snell2017prototypical} uses the support set to define a centroid $c_j$ for each class $j$ by averaging the features of the support examples belonging to class $j$:
\begin{equation*}
    c^{\Psi_{d^*}}_j = \frac{1}{|\mathcal{S}_{\mathcal{T}}^j|} \sum_{x \in \mathcal{S}_{\mathcal{T}}^j} f(x; \Phi, \Psi_{d^*})
\end{equation*}
where $\mathcal{S}_{\mathcal{T}}^j = \{ (x, y) \in \mathcal{S}_{\mathcal{T}}: y = j \}$ is the subset of the support set for class $j$. The $\Psi_{d^*}$ superscript in $c^{\Psi_{d^*}}_j$ serves to emphasize that the centroid was created from features  obtained by plugging in $\Psi_{d^*}$ into the shared template.

Under this classifier, the probability of an example $x$ belonging to class $j$ is proportional to the exponential of the cosine similarity between its features and that class centroid:
\begin{equation*}
    p^{\Psi_{d^*}}(j | x, \{ c^{\Psi_{d^*}}_j \}_{j=1}^N) \propto \exp  \frac{f(x; \Phi, \Psi_{d^*}) \cdot c^{\Psi_{d^*}}_j}{||f(x; \Phi, \Psi_{d^*})|| \cdot ||c^{\Psi_{d^*}}_j||}
\end{equation*}

% The cross-entropy loss of an example $(x^*, y^*)$ is then:
% \begin{equation*}
%     \mathcal{L}^{\Psi_{d^*}}(x^*, y^*, \{ c^{\Psi_{d^*}}_j \}_{j=1}^N) = - y^* \log p^{\Psi_{d^*}}(y^* | x^*, \{ c^{\Psi_{d^*}}_j \}_{j=1}^N)
% \end{equation*}

\paragraph{Learning the per-task parameters} We learn $\Psi_{d^*}$ via gradient descent to minimize the NCC loss on the support set:%\rz{Maybe we should switch learning to inferring here, or adapting, to make it clear that these are re-adapted each episode. And/or just state this more explicitly}
\begin{equation*}
    \Psi_{d^*} = \Psi_{d^*}^{init} - \epsilon \frac{\partial }{\partial \Psi_{d^*}}  \left(\sum_{(x, y) \in \mathcal{S}_\mathcal{T}} \mathcal{L}^{\Psi_{d^*}}(x, y, \{ c^{\Psi_{d^*}}_j \}_{j=1}^N)\right)
\end{equation*}
where $\epsilon$ is the learning rate and $\mathcal{L}^{\Psi_{d^*}}(x, y, \{ c^{\Psi_{d^*}}_j \}_{j=1}^N)$ denotes the cross-entropy loss for example $(x, y)$ under the NCC.
%\rz{This is the second definition of $\Psi_{d^*}$ -- it is defined with BLEND above. That one could be defined right away as the initial $\Psi_{d^*}$}
In practice, we might take more than a one step of gradient descent; we treat that as a hyperparameter. Note that all parameters aside from $\Psi_{d^*}$ are frozen at this time.

We also emphasize that we learn $\Psi_{d^*}$ on a per-task basis at test time, using the task's support set. That is, $\Psi_{d^*}$ is not re-used across the test tasks that are sampled from $d^*$.

\paragraph{Step 2: Predict a class label for each query example} Finally, having defined a feature extractor $f(\cdot ; \Phi, \Psi_{d^*})$ for the given test task, we can utilize the NCC to classify each query example. Concretely, we classify a query $x^*$ as:
\begin{equation*}
    \hat y^* = \argmax_{j} p^{\Psi_{d^*}}(j | x^*, \{ c^{\Psi_{d^*}}_j \}_{j=1}^N) 
\end{equation*}

==> FLUTE (ICML 2021)/source/preamble.tex <==
\usepackage{microtype}
\usepackage{graphicx}
\usepackage{subfigure}
\usepackage{booktabs}
\usepackage{hyperref}
\usepackage{datatool}
\usepackage{siunitx}

\usepackage{amsfonts}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{bbm}
\usepackage{bm}

\newcommand{\theHalgorithm}{\arabic{algorithm}}

\usepackage[
  % -- Uncomment for camera-ready --
   accepted
]{icml2021}

\icmltitlerunning{Learning a Universal Template for Few-shot Dataset Generalization \titlerunningsuffix}

\newcommand{\ra}[1]{\renewcommand{\arraystretch}{#1}}
\newcommand{\red}[1]{\textcolor{red}{#1}}
\newcommand{\green}[1]{\textcolor{green}{#1}}
\newcommand*\dtlformat[1]{\DTLifnumerical{#1}{\num{#1}}{#1}}

\DeclareMathOperator*{\argmax}{argmax}
\DeclareMathOperator*{\softmax}{softmax}
\DeclareMathOperator*{\onehot}{one-hot}
\newcommand{\model}{\textsc{FLUTE}}
\newcommand{\blend}{\textsc{BLEND}}

\DTLloaddb[noheader=true,omitlines=1]{example_table}{data/example_table.csv}
\DTLloaddb[noheader=true,omitlines=1]{all}{data/all.csv}
\DTLloaddb[noheader=true,omitlines=1]{ablations}{data/ablations.csv}

==> FLUTE (ICML 2021)/source/related_work.tex <==
\section{Related Work}
%The problem of few-shot dataset generalization is related to various well-studied areas: standard (single-dataset) few-shot classification, transfer learning, multi-task learning, and domain generalization. We first outline the similarities and differences from these related problems.
% \red{TODO: write high-level similarities and diffs compared to standard few-shot classification, transfer learning, multi-task learning and domain generalization.}
Few-shot dataset generalization is related to various well-studied areas. The aim in multi-task learning \cite{crawshaw2020multi}, for example, is to learn multiple tasks simultaneously with a shared model, similar to FLUTE's approach for training on multiple diverse datasets jointly. However, contray to that problem, our goal is to generalize to \emph{new datasets}. Domain generalization \cite{gulrajani2020search} also relates to our problem setting due to the shared goal of learning a model that generalizes to vastly different data distributions, but it typically assumes that the label space is shared across datasets, contrary to our setting.

Another related area is transfer learning \cite{zhuang2020comprehensive}, aiming to improve a learner's performance on target domains via leveraging knowledge obtained from related source domains. A representative approach that is related to FLUTE is that of \citet{puigcerver2021scalable}: they first train a set of diverse `experts' on different data and then, for each downstream task, they select the most appropriate expert and fine-tune it on that task. FLUTE differs in that, thanks to its universal template that can be re-used across tasks of different datasets, it only needs to fine-tune a small number of per-task parameters at test time (the FiLM parameters); a design that allows to effectively leverage previous knowledge and avoid overfitting in our data-scarce setting.

Moreover, FLUTE is related to several few-shot learning methods. Many popular ones are metric-based \cite{vinyals2016matching,snell2017prototypical,sung2018learning}, or learning-to-learn approaches \cite{ravi2016optimization,finn2017model}. A particular variant of the influential Model Agnostic Meta Learning (MAML) model that is especially related to FLUTE is CAVIA \cite{zintgraf2019fast} that also divides the feature extractor's parameters into task-general and task-specific ones. At test time, only the task-specific ones are adapted for each new episode. Moreover, \citep{flennerhag2019meta} propose to interleave meta-learned `warp-layers' between the layers of a task learner, in the context of gradient-based meta-learning. Reminiscent of FLTUE's template, their warp-layers are shared across tasks, with the aim in that case being to efficiently parameterize a preconditioning matrix that facilitates within-task learning. Albeit related, these previous approaches do not target our across-dataset problem setting of interest, and differ algorithmically as they utilize a meta-learning approach, whereas FLUTE is trained across datasets, with the simple training objective of joint dataset classification. Keeping with the spirit of separating shared from specific weights, \citep{wang2019meta} design a model for few-shot object detection based on the insight of disentangling category-specific and category-agnostic parameters, in a similar spirit to FLUTE's dataset-specific and dataset-agnostic parameters.  However, their approach differs significantly on an architectural level, as well as in terms of their training objective and overall goal and application area of the work.

FiLM has also been used in several few-shot learning approaches, typically for the purpose of conditioning on each episode's support set to construct a set of features that are tailored to the task at hand \cite{oreshkin2018tadam,requeima2019fast,bateni2019improved}. FLUTE differs from these works in that, consistent with its goal of constructing a dataset-general template, it conditions on the dataset label, instead of conditioning on a continuous representation of support-set features as those previous works. This idea relates to \cite{rebuffi2017learning}'s work that introduce `residual adapters', a generalization of FiLM, to condition on different datasets. However, that work does not consider the problem that is our focus: generalization to new datasets at test time.
% Briefly, CAVIA and Wang et al. (2019) also separate ``general'' and ``specific'' parameters, but both their training objectives for learning those and their end-goals are very different from ours. FLUTE is specifically designed and makes important progress for few-shot dataset generalization. Rebuffi et al. (2017) use a similar architecture, but don't consider the problem that is our focus: generalization to new datasets.

The idea of using a dataset classifier in the Blender network to guide the initializaiton of new sets of FiLM parameters is reminiscent of \cite{torralba2011unbiased}'s earlier work, where they noticed that it is possible to accurately classify datasets, suggesting that each has a unique “signature”.

Finally, perhaps the most closely-related family of work is that of building a \emph{universal representation}; a term coined in \citet{bilen2017universal} to describe a set of rich features that enable strong performance on several different datasets in a multi-task learning setup. Building on this idea, the approach of Selecting from a Universal Representation (SUR \citep{dvornik2020selecting}) achieved strong performance by training a separate feature extractor on each training dataset (for a total of $M$ extractors). To tackle each test task, they obtain the $M$ sets of extracted features for the task's data, and concatenate them to form a universal representation of size $MD$, where $D$ is the representation size of each feature extractor. They then utilize a selection mechanism that weights these $MD$ features based on relevance to the task at hand. \citet{liu2020universal} later improved upon SUR by replacing its feature weighting mechanism by a meta-learned attention layer referred to as the Universal Representation Transformer layer (URT). To alleviate the cost of training $M$ separate feature extractors, SUR and URT offer `paramteric family' variants, SUR-pf and URT-pf, respectively, where their $M$ feature extractors share all but their batch normalization weights; a design that is architecturally similar to FLUTE's. Unfortunately, though, the compactness of SUR-pf/URT-pf results in %costs them 
a significant drop in accuracy.

Compared to those works, FLUTE embodies a different inductive bias: we don't seek a set of universal features from which we select dataset-relevant ones. Instead, we seek a universal template that defines several dataset-specialized feature extractors, each of which only produces dataset-relevant features. An additional difference is that SUR-pf/URT-pf train the shared parameters only on ImageNet, whereas we employ a joint training phase that permits all datasets to influence those parameters; a choice that 
%we hypothesize and examine empirically 
is crucial for turning the shared parameters into a general-purpose universal template. Finally, FLUTE scales better with the number of training datasets, as summarized in Table~\ref{table:flute_vs_sur_urt}.%, in terms of several aspects: number of parameters, representation size, and amount of computation required for each task. We summarize these differences in Table~\ref{table:flute_vs_sur_urt}.

\begin{table}[ht]
	\ra{1.2}
	\caption{\label{table:flute_vs_sur_urt} Comparing FLUTE to universal representation methods in terms of scalability with the number $M$ of training datasets. $P$ is the number of feature extractor parameters, $D$ the size of representation that the feature extractor outputs (e.g. 512 for a ResNet-18), $H$ the number of URT's attention heads and $T$ the number of FLUTE's within-task training steps to learn $\Psi_h$ during evaluation. `Computation' measures the number of passes through the feature extractor(s) for each task. SUR(-pf) and URT(-pf) forward-pass through their $M$ extractors (some of which share parameters in the pf variants) whereas we only maintain a single feature extractor. We perform a forward and a backward pass on the support set for each of our $T$ steps, and a final forward pass on the query set ($2T+1$ in total); thus FLUTE's amount of test-time computation %\rz{Should make clear Computation refers to evaluation, not learning.} 
		does \emph{not} grow with the number of training datasets as for SUR(-pf) and URT(-pf), and $T$ can be small in practice.}
	\begin{center}
		\begin{tabular}{lccc}
			\toprule
			& Num params & Size of repr. & Computation \\
			SUR & $MP$ & $MD$ & $M$\\
			URT & $MP$ & $HD$ & $M$\\
			SUR-pf & $P$ & $MD$ & $M$\\
			URT-pf & $P$ & $HD$ & $M$\\
			FLUTE & $P$ & $D$ & $2T+1$\\
			\bottomrule
		\end{tabular}
	\end{center}
\end{table}

% \red{TODO: WRITEME.}
% \red{Things to mention:
% \begin{itemize}
%     \item Relationship with SUR and URT
%     \item Relationship with transfer learning approaches: our approach is not trained episodically, and is better described as a transfer learning approach which leverages the shared parameterization of a family of classifiers for initialization.
%     \item Relationship with \citet{puigcerver2021scalable}'s experts mixture approach: they also train a parametric
% \end{itemize}}


==> FLUTE (ICML 2021)/source/results.tex <==
\section{Results}

\begin{table*}
\ra{1.2}
\caption{\label{table:main} Comparison of FLUTE to the previous state-of-the-art approaches on Meta-Dataset. The few-shot dataset generalization performance is shown in the second group of rows (Traffic Signs - CIFAR-100), representing unseen datasets that require Strong Generalization (SG). For completeness, we also present results on the easier problem of Weak Generalization (WG) in the first 8 rows (ImageNet - Flower). We compare against CNAPs \cite{requeima2019fast}, TaskNorm \cite{bronskill2020tasknorm}, SimpleCNAPS \cite{bateni2019improved}, SUR(-pf) \cite{dvornik2020selecting} and URT(-pf) \cite{liu2020universal}. We emphasize that SUR and URT have 8 times more parameters compared to all other competitors (denoted by x8). FLUTE outperforms these previous methods by a significant margin for the problem of few-shot dataset generalization ($>5\%$ on Average SG) while still outperforming the state-of-the-art overall.}
\begin{center}
\scriptsize
\begin{tabular}{@{}lcccccccc@{}}
  \toprule
  Dataset & CNAPs & TaskNorm & SimpleCNAPs & SUR-pf & URT-pf & SUR (x8) & URT (x8) & FLUTE \\
  \midrule
  \DTLforeach{all}{%
    \task=Column1,%
    \avgI=Column2,%
    \ciI=Column3,%
    \avgII=Column4,%
    \ciII=Column5,%
    \avgIII=Column6,%
    \ciIII=Column7,%
    \avgIX=Column8,%
    \ciIX=Column9,%
    \avgX=Column10,%
    \ciX=Column11,%
    \avgXI=Column12,%
    \ciXI=Column13,%
    \avgXII=Column14,%
    \ciXII=Column15,%
    \avgXIII=Column16,%
    \ciXIII=Column17%
  }{%
    \ifthenelse{\value{DTLrowi}=1}{}{%
      \ifthenelse{\value{DTLrowi}=9 \OR \value{DTLrowi}=14}{\\\midrule}{\\}%
    }%
    \dtlformat{\task}&%
    \dtlformat{\avgI} \ifthenelse{\value{DTLrowi}>13}{}{$\pm$ \dtlformat{\ciI}}\%&%
    \dtlformat{\avgII} \ifthenelse{\value{DTLrowi}>13}{}{$\pm$ \dtlformat{\ciII}}\%&%
    \dtlformat{\avgIII} \ifthenelse{\value{DTLrowi}>13}{}{$\pm$ \dtlformat{\ciIII}}\%&%
    \dtlformat{\avgIX} \ifthenelse{\value{DTLrowi}>13}{}{$\pm$ \dtlformat{\ciIX}}\%&%
    \dtlformat{\avgX} \ifthenelse{\value{DTLrowi}>13}{}{$\pm$ \dtlformat{\ciX}}\%&%
    \dtlformat{\avgXI} \ifthenelse{\value{DTLrowi}>13}{}{$\pm$ \dtlformat{\ciXI}}\%&%
    \dtlformat{\avgXII} \ifthenelse{\value{DTLrowi}>13}{}{$\pm$ \dtlformat{\ciXII}}\%&%
    \dtlformat{\avgXIII} \ifthenelse{\value{DTLrowi}>13}{}{$\pm$ \dtlformat{\ciXIII}}\%%
  }
  \\\bottomrule
\end{tabular}
\end{center}
\end{table*}

\paragraph{Performance on Meta-Dataset} As our first experiment, we evaluate FLUTE on Meta-Dataset, in order to assess its performance on the challenging problem of few-shot dataset generalization, as well as on the weaker generalization setup. We compare against previous approaches that have the same number of parameters as FLUTE, as well as the state-of-the-art models on Meta-Dataset that use roughly 8 times more parameters than FLUTE. We present these results in Table~\ref{table:main}. We observe that FLUTE significantly outperforms all approaches on few-shot dataset generalization. Overall, it sets the new state-of-the-art on Meta-Dataset, despite FLUTE's compactness and parameter efficiency.
%\rz{This is the main result of the paper. It would be nice to figure out some way of bringing this out more. As it stands it is mentioned here and then you dive right into analysis and ablations.}\et{I totally agree. Let me know everyone if you have any suggestions on how to do this, I'm struggling to find a way to place more emphasis on this without taking up too much space.}

Having established FLUTE's effectiveness, we next take a closer look at the effect of its various design choices. %We also include additional analyses in the Appendix.
\begin{table}[h]
\ra{1.2}
\caption{\label{table:ablations_wo_ci} The effect of training on different data (`All', as in FLUTE, or `ImageNet-only'), and alternative initialization schemes for $\Psi_{d^*}$: from scratch (`scratch') and from ImageNet's FiLM parameters (`$\Psi_{IN}$'). The first column is the FLUTE model. We include confidence intervals for this table in the Appendix.}
\begin{center}
\scriptsize
\begin{tabular}{@{}l|c|cc|cc@{}}
\toprule
\multicolumn{1}{l}{Training data} & \multicolumn{1}{c}{All} & \multicolumn{2}{c}{All} & \multicolumn{2}{c}{ImageNet only} \\
\multicolumn{1}{l}{Init scheme} & Blender & Scratch & $\Psi_{IN}$ & Scratch & $\Psi_{IN}$\\
\midrule
\DTLforeach{ablations}{%
  \task=Column1,%
  \avgI=Column2,%
  \ciI=Column3,%
  \avgII=Column4,%
  \ciII=Column5,%
  \avgIII=Column6,%
  \ciIII=Column7,%
  \avgIX=Column8,%
  \ciIX=Column9,%
  \avgX=Column10,%
  \ciX=Column11,%
  \avgXI=Column12,%
  \ciXI=Column13%
}{%
  \ifthenelse{\value{DTLrowi}=1}{}{%
    \ifthenelse{\value{DTLrowi}=9 \OR \value{DTLrowi}=14}{\\\midrule}{\\}%
  }%
  \dtlformat{\task}&%
  \dtlformat{\avgI} \ifthenelse{\value{DTLrowi}>13}{}{}\%&%
%   \dtlformat{\avgXI} \ifthenelse{\value{DTLrowi}>13}{}{}\%&%
  \dtlformat{\avgII} \ifthenelse{\value{DTLrowi}>13}{}{}\%&%
  \dtlformat{\avgIII} \ifthenelse{\value{DTLrowi}>13}{}{}\%&%
  \dtlformat{\avgIX} \ifthenelse{\value{DTLrowi}>13}{}{}\%&%
  \dtlformat{\avgX} \ifthenelse{\value{DTLrowi}>13}{}{}\%%
%   \dtlformat{\avgXI} \ifthenelse{\value{DTLrowi}>13}{}{}\%%
}
\\\bottomrule
\end{tabular}
\end{center}
\end{table}

\paragraph{The importance of the Blender network} Recall that the role of this network is to propose an initialization for the FiLM parameters for each test task. We now explore two alternative ways of initializing those parameters: `from scratch' and `from ImageNet' ($\Psi_{IN}$). For each layer $i$, the former sets the additive terms $\beta_i$ to vectors of 0s, and the multiplicative terms $\gamma_i$ to vectors of 1s, while the latter sets the FiLM parameters throughout the network to those learned specifically for the ImageNet dataset, which we denote by $\Psi_{IN}$. We singled out ImageNet for this since it is often treated as a good source for transfer.

The results for this experiment are shown in the second and third  columns of Table~\ref{table:ablations_wo_ci} (the first shows FLUTE for reference). We find that initializing from $\Psi_{IN}$ yields impressive results on several datasets (e.g. ImageNet (unsurprisingly), but also Textures, CIFAR-10, CIFAR-100) but very poor results on datasets that are vastly different from ImageNet (e.g. Omiglot, Quickdraw, and Aircraft). On the other hand, initializing from scratch does not recover that strong performance on the ImageNet-like datasets, but evidently constitutes a much better solution for various other datasets (e.g. Omniglot, Quickraw and Aircraft). Therefore, the initialization of $\Psi_{d^*}$ really matters, with different techniques working best for different evaluation datasets. Our Blender network thus provides a good solution by tailoring the initialization to each task at hand, via the predicted compatibility with each training dataset.

\begin{figure*}[t]%
    \centering%
    \includegraphics[height=2.1cm]{figures/cifar10.pdf}%
    \includegraphics[height=2.1cm]{figures/cifar100.pdf}%
    \includegraphics[height=2.1cm]{figures/unshuffled_traffic_sign.pdf}%
    \includegraphics[height=2.1cm]{figures/mnist.pdf}%
    \includegraphics[height=2.1cm]{figures/mscoco.pdf}%
    \caption{The support and query accuracy over 600 test episodes of unseen datasets as a function of the fine-tuning steps for $\Psi_{d^*}$.}%
    \label{fig:fine_tuning}%
\end{figure*}

\paragraph{The importance of diverse training data}  Next, we empirically examine our hypothesis that training our feature extractor on \emph{all} training datasets is an important choice for encouraging (the convolutional layers of) our feature extractor to act as a universal template. In other words, had we not trained it on diverse data, perhaps it would be less general and thus less capable of supporting generalization to new datasets via merely changing the values of the batch normalization parameters. To investigate this, we trained a feature extractor (of identical architecture to FLUTE's) on ImageNet only. In this case, we only learn one set of FiLM parameters during training, since there is only one training dataset. We then attempt to tackle the test tasks similarly to FLUTE, by learning a new set of FiLM parameters for each, via one of the two initialization schemes proposed in the previous round of experiments.

The results produced by this ImageNet-only feature extractor are shown in the last two columns of Table~\ref{table:ablations_wo_ci}. We find that the feature extractor trained on all datasets performs significantly better across the board compared to that trained on ImageNet only, validating our hypothesis. Between the two initialization methods for the ImageNet-trained feature extractor, we still observe certain trade-offs like the ones identified for FLUTE's feature extractor, but notably, `from scratch' no longer performs well for datasets like Omniglot and Quickdraw as before. This speaks to the inferior generalizability of this feature extractor that was trained on less diverse data. Finally, we observe that even when evaluating on test classes from ImageNet (first row), FLUTE's feature extractor evidently constitutes a better template compared to the ImageNet-trained one, indicating positive transfer during FLUTE's multi-tasking training phase.

\begin{figure}%
    \centering%
    \includegraphics[width=\linewidth]{figures/heatmap.pdf}%
    \caption{\label{fig:heatmap} Visualization of the coefficients of the convex combination produced by the Blender network for various test datasets. Each column represents the average coefficients produced for 600 test tasks of a particular dataset.}%
\end{figure}

\paragraph{The effect of the number of steps to train $\Psi_{d^*}$} Figure~\ref{fig:fine_tuning} plots the support and query accuracy during the fine-tuning of the per-task parameters $\Psi_{d^*}$ on the support set, averaged over 600 test tasks of each unseen domain (strong generalization setting). We also show the corresponding plots for weak generalization in the Appendix. We used 6 steps for this, with a learning rate of 0.005, which are the values we used for FLUTE's results in Table~\ref{table:main}, chosen based on the validation set. We observe that some datasets benefit more than others from this fine-tuning. In fact, in some cases (CIFAR-100, MSCOCO) the support accuracy even decreases. This indicates that perhaps those hyperparameters aren't ideal for all test tasks. Moreover, the validation set may not be a good proxy for the test set, since it is comprised of different datasets, making hyperparameter selection hard. Tailoring the learning rate or number of steps to each task would be an interesting avenue for future work.  %Therefore, it is possible that a more aggressive learning rate would yield better results on episodes of held-out datasets. 
%We believe that discovering an appropriate model selection approach in this non-i.i.d. setting is an interesting direction for future work. 

\paragraph{Inspecting the Blender's proposals} We visualize the combination coefficients that the Blender produces for test tasks in Figure~\ref{fig:heatmap}. We notice that for test episodes of datasets seen during training (weak generalization setting), the Blender very strongly selects the dataset from which the task originated. For new datasets that did not appear in the training set (last 5 columns), the Blender seems to make reasonable choices (e.g. Quickdraw for MNIST, ImageNet for MSCOCO) but the probability distribution may be less peaky (e.g. for Traffic Signs and CIFAR-100). In the Appendix we also investigate the variance of these predictions across different test tasks within each dataset.
% \rz{Can we add a pointer to examining variance issue in Appendix?}

%\rz{One more general issue comes to mind here -- it is unclear what makes the method specific to dataset generalization. The UT parameters are initialized and adapted based on the support set in an episode. So they need not be consistent across episodes of a given dataset. The Blender is defined as a mixture across training datasets. Fig 2 shows the coefficients for test and train datasets. How much do these vary across episodes?}\et{Exactly, our method isn't specific to few-shot dataset generalization - it can also handle the weaker generalization problem of held-out classes of seen datasets. I was emphasizing dataset generalization throughout the paper in particular because that's the setting where we get the largest win compared to previous methods. :-) but let me know if you find this misleading? I find that the co-efficients are very consistent for seen datasets, and vary a bit more for unseen ones. Maybe we can add a visualization of the variance of these co-efficients for different datasets in the Appendix. What do you think?}.


\paragraph{Discussion} As alluded to earlier, an open challenge is defining an appropriate model selection mechanism for the difficult scenario when the provided validation set is not a good proxy for the test set. The problem that we study in this work, similarly to domain generalization \cite{gulrajani2020search},
%\rz{This paper has an extensive discussion of this issue} 
suffers from underspecification: there may be several solutions that all perform well on the training and validation sets but behave differently on the test set. With this in mind, perhaps we should adjust our evaluation metrics to account for this potential source of variance. For instance, in the context of FLUTE, we noticed in Table~\ref{table:ablations_wo_ci} that the initialization of $\Psi_{d^*}$ really matters, therefore perhaps the results are sensitive to the chosen checkpoint of the dataset classifier. We report in the Appendix the performance across more runs of that component and observe some variance on held-out datasets, but our conclusions hold across runs.

==> FLUTE (ICML 2021)/source/results_expanded.tex <==
\section{Results}

\begin{table*}
\ra{1.2}
\caption{\label{table:main} Comparison of FLUTE to the previous state-of-the-art approaches on Meta-Dataset. The few-shot dataset generalization performance is shown in the second group of rows (Traffic Signs - CIFAR-100), representing unseen datasets that require Strong Generalization (SG). For completeness, we also present results on the easier problem of Weak Generalization (WG) in the first 8 rows (ImageNet - Flower). We compare against CNAPs \cite{requeima2019fast}, TaskNorm \cite{bronskill2020tasknorm}\footnotemark, SimpleCNAPS \cite{bateni2019improved}, SUR(-pf) \cite{dvornik2020selecting} and URT(-pf) \cite{liu2020universal}. We emphasize that SUR and URT have 8 times more parameters compared to all other competitors (denoted by x8). FLUTE outperforms these previous methods by a significant margin for the problem of few-shot dataset generalization ($>5\%$ on Average SG) while still outperforming the state-of-the-art overall. Each number represents the average query set accuracy over 600 test tasks, and its 95\% confidence interval.}
\begin{center}
\scriptsize
\begin{tabular}{@{}lcccccccc@{}}
  \toprule
  Dataset & CNAPs & TaskNorm & SimpleCNAPs & SUR-pf & URT-pf & SUR (x8) & URT (x8) & FLUTE \\
  \midrule
  \DTLforeach{all_correct_TS}{%
    \task=Column1,%
    \avgI=Column2,%
    \ciI=Column3,%
    \avgII=Column4,%
    \ciII=Column5,%
    \avgIII=Column6,%
    \ciIII=Column7,%
    \avgIX=Column8,%
    \ciIX=Column9,%
    \avgX=Column10,%
    \ciX=Column11,%
    \avgXI=Column12,%
    \ciXI=Column13,%
    \avgXII=Column14,%
    \ciXII=Column15,%
    \avgXIII=Column16,%
    \ciXIII=Column17%
  }{%
    \ifthenelse{\value{DTLrowi}=1}{}{%
      \ifthenelse{\value{DTLrowi}=9 \OR \value{DTLrowi}=14}{\\\midrule}{\\}%
    }%
    \dtlformat{\task}&%
    \dtlformat{\avgI} \ifthenelse{\value{DTLrowi}>13}{}{$\pm$ \dtlformat{\ciI}}&%
    \dtlformat{\avgII} \ifthenelse{\value{DTLrowi}>13 \OR \value{DTLrowi}=9}{}{$\pm$ \dtlformat{\ciII}}&%
    \dtlformat{\avgIII} \ifthenelse{\value{DTLrowi}>13}{}{$\pm$ \dtlformat{\ciIII}}&%
    \dtlformat{\avgIX} \ifthenelse{\value{DTLrowi}>13}{}{$\pm$ \dtlformat{\ciIX}}&%
    \dtlformat{\avgX} \ifthenelse{\value{DTLrowi}>13}{}{$\pm$ \dtlformat{\ciX}}&%
    \dtlformat{\avgXI} \ifthenelse{\value{DTLrowi}>13}{}{$\pm$ \dtlformat{\ciXI}}&%
    \dtlformat{\avgXII} \ifthenelse{\value{DTLrowi}>13}{}{$\pm$ \dtlformat{\ciXII}}&%
    \dtlformat{\avgXIII} \ifthenelse{\value{DTLrowi}>13}{}{$\pm$ \dtlformat{\ciXIII}}%
  }
  \\\bottomrule
\end{tabular}
\end{center}
\end{table*}

\paragraph{Performance on Meta-Dataset} As our first experiment, we evaluate FLUTE on Meta-Dataset, in order to assess its performance on the challenging problem of few-shot dataset generalization, as well as on the weaker generalization setup. We compare against previous approaches that have the same number of parameters as FLUTE, as well as the state-of-the-art models on Meta-Dataset that use roughly 8 times more parameters than FLUTE. We present these results in Table~\ref{table:main}. We observe that FLUTE significantly outperforms all approaches on few-shot dataset generalization. Overall, it sets the new state-of-the-art on Meta-Dataset, despite FLUTE's compactness and parameter efficiency.
%\rz{This is the main result of the paper. It would be nice to figure out some way of bringing this out more. As it stands it is mentioned here and then you dive right into analysis and ablations.}\et{I totally agree. Let me know everyone if you have any suggestions on how to do this, I'm struggling to find a way to place more emphasis on this without taking up too much space.}

Having established FLUTE's effectiveness, we next take a closer look at the effect of its various design choices. \footnotetext{We don't report Traffic Signs results for this method due to an inconsistency in how evaluation on this dataset was performed (described in the Appendix)}

\begin{table}[h]
\ra{1.2}
\caption{\label{table:ablations_wo_ci} The effect of training on different data (`All', as in FLUTE, or `ImageNet-only'), and alternative initialization schemes for $\Psi_{d^*}$: from scratch (`Scratch'), from ImageNet's FiLM parameters (`$\Psi_{IN}$') and from Blender. The column corresponding to the setting ``All, Blender'' is our proposed FLUTE model. Each number represents the average query set accuracy over 600 test tasks, and its 95\% confidence interval. We include confidence intervals for this table in the Appendix.}
\begin{center}
\scriptsize
\begin{tabular}{@{}l|ccc|ccc@{}}
\toprule
\multicolumn{1}{l}{Training data} & \multicolumn{3}{c}{All} & \multicolumn{3}{c}{ImageNet only} \\
\multicolumn{1}{l}{Init scheme} & Scratch & $\Psi_{IN}$ & Blender & Scratch & $\Psi_{IN}$ & Blender \\
\midrule
\DTLforeach{ablations_correct_TS}{%
  \task=Column1,%
  \avgI=Column2,%
  \ciI=Column3,%
  \avgII=Column4,%
  \ciII=Column5,%
  \avgIII=Column6,%
  \ciIII=Column7,%
  \avgIX=Column8,%
  \ciIX=Column9,%
  \avgX=Column10,%
  \ciX=Column11,%
  \avgXI=Column12,%
  \ciXI=Column13%
}{%
  \ifthenelse{\value{DTLrowi}=1}{}{%
    \ifthenelse{\value{DTLrowi}=9 \OR \value{DTLrowi}=14}{\\\midrule}{\\}%
  }%
  \dtlformat{\task}&%
%   \dtlformat{\avgXI} \ifthenelse{\value{DTLrowi}>13}{}{}\%&%
  \dtlformat{\avgII} \ifthenelse{\value{DTLrowi}>13}{}{}&%
  \dtlformat{\avgIII} \ifthenelse{\value{DTLrowi}>13}{}{}&%
  \dtlformat{\avgI} \ifthenelse{\value{DTLrowi}>13}{}{}&%
  \dtlformat{\avgIX} \ifthenelse{\value{DTLrowi}>13}{}{}&%
  \dtlformat{\avgX} \ifthenelse{\value{DTLrowi}>13}{}{}&%
  \dtlformat{\avgXI} \ifthenelse{\value{DTLrowi}>13}{}{}%
}
\\\bottomrule
\end{tabular}
\end{center}
\end{table}

\paragraph{The importance of the Blender network} Recall that the role of this network is to propose an initialization for the FiLM parameters for each test task. We now explore two alternative ways of initializing those parameters: `from scratch' and `from ImageNet' ($\Psi_{IN}$). For each layer $i$, the former sets the additive terms $\beta_i$ to vectors of 0s, and the multiplicative terms $\gamma_i$ to vectors of 1s, while the latter sets the FiLM parameters throughout the network to those learned specifically for the ImageNet dataset, which we denote by $\Psi_{IN}$. We singled out ImageNet for this since it is often treated as a good source for transfer.

The results for this experiment are shown in the first three columns of Table~\ref{table:ablations_wo_ci}. We find that initializing from $\Psi_{IN}$ yields impressive results on several datasets (e.g. ImageNet (unsurprisingly), but also Textures, CIFAR-10, CIFAR-100) but very poor results on datasets that are vastly different from ImageNet (e.g. Omiglot, Quickdraw, and Aircraft). On the other hand, initializing from scratch does not recover that strong performance on the ImageNet-like datasets, but evidently constitutes a much better solution for various other datasets (e.g. Omniglot, Quickraw and Aircraft). Therefore, the initialization of $\Psi_{d^*}$ really matters, with different techniques working best for different evaluation datasets. Our Blender network thus provides a good solution by tailoring the initialization to each task at hand, via the predicted compatibility with each training dataset.

\begin{figure*}[t]%
    \centering%
    \includegraphics[height=2.1cm]{figures/cifar10.pdf}%
    \includegraphics[height=2.1cm]{figures/cifar100.pdf}%
    \includegraphics[height=2.1cm]{figures/unshuffled_traffic_sign.pdf}%
    \includegraphics[height=2.1cm]{figures/mnist.pdf}%
    \includegraphics[height=2.1cm]{figures/mscoco.pdf}%
    \caption{The support and query accuracy over 600 test episodes of unseen datasets as a function of the fine-tuning steps for $\Psi_{d^*}$.}%
    \label{fig:fine_tuning}%
\end{figure*}

\paragraph{The importance of diverse training data}  Next, we empirically examine our hypothesis that training our feature extractor on \emph{all} training datasets is an important choice for encouraging (the convolutional layers of) our feature extractor to act as a universal template. In other words, had we not trained it on diverse data, we hypothesize it would be less general and thus less capable of supporting generalization to new datasets via merely changing the values of the batch normalization parameters. To investigate this, we trained a feature extractor (of identical architecture to FLUTE's) on ImageNet only. In this case, we only learn one set of FiLM parameters during training, since there is only one training dataset. We then attempt to tackle the test tasks similarly to FLUTE, by learning a new set of FiLM parameters for each, via one of the three initialization schemes proposed in the previous round of experiments.

In order to be able to use the Blender heuristic with this feature extractor too, we require a set of FiLM parameters for each of the training datasets. For the ImageNet dataset, we already have this: the FiLM parameters correspond to the batch normalization parameters obtained when training this feature extractor on ImageNet. For each of the remaining training datasets, we launch a training phase to learn a new set of batch normalization parameters, keeping the convolutional parameters frozen to those learned by this ImageNet-only feature extractor. This is reminiscent of SUR-pf's procedure for learning batch normalization parameters for the different training datasets, for use with an ImageNet-trained feature extractor. Once we have obtained the FiLM parameters for each of the training datasets for this ImageNet feature extractor, we use our dataset classifier within Blender to obtain the initialization of $\Psi_{d^*}$ as usual.

The performance of this ImageNet-only feature extractor, with different initialization heuristics for $\Psi_{d^*}$, are shown in the last three columns of Table~\ref{table:ablations_wo_ci}. We find that, for any given initialization heuristic, the feature extractor trained on all datasets performs significantly better across the board compared to that trained on ImageNet only, validating our hypothesis. 
%Between the two initialization methods for the ImageNet-trained feature extractor, we still observe certain trade-offs like the ones identified for FLUTE's feature extractor, but notably, `from scratch' no longer performs well for datasets like Omniglot and Quickdraw as before. This speaks to the inferior generalizability of this feature extractor that was trained on less diverse data.
Notably, the `Scratch' heuristic no longer performs well for datasets like Omniglot and Quickdraw, as it did when using FLUTE's feature extractor. This speaks to the inferior generalizability of this feature extractor that was trained on less diverse data. 
Finally, we observe that even when evaluating on test classes from ImageNet (first row), FLUTE's feature extractor evidently constitutes a better template compared to the ImageNet-trained one, indicating positive transfer during FLUTE's joint training phase.

\paragraph{The effect of the number of steps to train $\Psi_{d^*}$} Figure~\ref{fig:fine_tuning} plots the support and query accuracy during the fine-tuning of the per-task parameters $\Psi_{d^*}$ on the support set, averaged over 600 test tasks of each unseen domain (strong generalization setting). We also show the corresponding plots for weak generalization in the Appendix. We used 6 steps for this, with a learning rate of 0.005, which are the values we used for FLUTE's results in Table~\ref{table:main}, chosen based on the validation set. We observe that some datasets benefit more than others from this fine-tuning. In fact, in some cases (CIFAR-100, MSCOCO) the support accuracy even decreases. This indicates that perhaps those hyperparameters aren't ideal for all test tasks. Moreover, the validation set may not be a good proxy for the test set, since it is comprised of different datasets, making hyperparameter selection hard. Tailoring the learning rate or number of steps to each task would be an interesting avenue for future work.  %Therefore, it is possible that a more aggressive learning rate would yield better results on episodes of held-out datasets. 
%We believe that discovering an appropriate model selection approach in this non-i.i.d. setting is an interesting direction for future work. 

\paragraph{Inspecting the Blender's proposals} We visualize the combination coefficients that the Blender produces for test tasks in Figure~\ref{fig:heatmap}. We notice that for test episodes of datasets seen during training (weak generalization setting), the Blender very strongly selects the dataset from which the task originated. For new datasets that did not appear in the training set (last 5 columns), the Blender seems to make reasonable choices (e.g. Quickdraw for MNIST, ImageNet for MSCOCO) but the probability distribution may be less peaky (e.g. for Traffic Signs and CIFAR-100). In the Appendix we also investigate the variance of these predictions across different test tasks within each dataset.

\begin{figure}%
    \centering%
    \includegraphics[width=\linewidth]{figures/heatmap.pdf}%
    \caption{\label{fig:heatmap} Visualization of the coefficients of the convex combination produced by the Blender network for various test datasets. Each column represents the average coefficients produced for 600 test tasks of a particular dataset.}%
\end{figure}

\paragraph{The effect of taking a convex combination} Having inspected the combination weights that Blender produces, we noticed that it often relies almost exclusively on a single dataset's FiLM parameters to form the initialization of the FiLM parameters of a new task. A natural question to ask, therefore, is whether the convex combination is required. An alternative design choice is a `Hard Blender' that selects only the FiLM parameters of the most compatible training dataset (as assessed by the dataset classifier), instead of combining them all in a weighted manner. We provide a detailed comparison with this variant in Table~\ref{table:hard_blender_comparison} in the Appendix. Indeed, the two initialization schemes perform similarly, especially on weak generalization tasks, where the Blender's co-efficients already resemble a hard selection. We observe, though, that the combination approach may yield small gains on strong generalization tasks. Overall, since Blender is a more general approach and it may improve the performance on new datasets, we adopt this initialization scheme as our default one for FLUTE.

% \rz{Can we add a pointer to examining variance issue in Appendix?}
%\rz{One more general issue comes to mind here -- it is unclear what makes the method specific to dataset generalization. The UT parameters are initialized and adapted based on the support set in an episode. So they need not be consistent across episodes of a given dataset. The Blender is defined as a mixture across training datasets. Fig 2 shows the coefficients for test and train datasets. How much do these vary across episodes?}\et{Exactly, our method isn't specific to few-shot dataset generalization - it can also handle the weaker generalization problem of held-out classes of seen datasets. I was emphasizing dataset generalization throughout the paper in particular because that's the setting where we get the largest win compared to previous methods. :-) but let me know if you find this misleading? I find that the co-efficients are very consistent for seen datasets, and vary a bit more for unseen ones. Maybe we can add a visualization of the variance of these co-efficients for different datasets in the Appendix. What do you think?}.


\paragraph{Discussion} As alluded to earlier, an open challenge is defining an appropriate model selection mechanism for the difficult scenario when the provided validation set is not a good proxy for the test set. The problem that we study in this work, similarly to domain generalization \cite{gulrajani2020search},
%\rz{This paper has an extensive discussion of this issue} 
suffers from underspecification: there may be several solutions that all perform well on the training and validation sets but behave differently on the test set. With this in mind, perhaps we should adjust our evaluation metrics to account for this potential source of variance. For instance, in the context of FLUTE, we noticed in Table~\ref{table:ablations_wo_ci} that the initialization of $\Psi_{d^*}$ really matters, therefore perhaps the results are sensitive to the chosen checkpoint of the dataset classifier. We report in the Appendix the performance across more runs of that component and observe some variance on held-out datasets, but our conclusions hold across runs.

==> FLUTE (ICML 2021)/source/title.tex <==
\twocolumn[
  % TODO(vdumoulin): Find a better title
%   \icmltitle{\titleprefix SURFiLM'n U.S.A \red{TODO: change me}}
  \icmltitle{\titleprefix Learning a Universal Template for Few-shot Dataset Generalization}
  \icmlsetsymbol{equal}{*}
  
  \begin{icmlauthorlist}
  % TODO(vdumoulin): change author list to the order we end up deciding.
  \icmlauthor{Eleni Triantafillou}{vector,google,atGoogle}
  \icmlauthor{Hugo Larochelle}{google}
  \icmlauthor{Richard Zemel}{vector}
\icmlauthor{Vincent Dumoulin}{google}
  \end{icmlauthorlist}
  
  \icmlaffiliation{google}{Google Research, Brain Team}
  \icmlaffiliation{vector}{University of Toronto, Vector Institute}
  \icmlaffiliation{atGoogle}{Work done at Google.}
  
  \icmlcorrespondingauthor{Eleni Triantafillou}{eleni@cs.toronto.edu}
  
  \icmlkeywords{Machine Learning, ICML, Few-Shot Classification}
  
  \vskip 0.3in
]

\printAffiliationsAndNotice{}


==> FLUTE (ICML 2021)/tables/ablations.tex <==
{\onecolumn
  \begin{table}[ht]
  \ra{1.2}
  \caption{\label{table:all} All.}
  \begin{center}
  \scriptsize
  \begin{tabular}{@{}lcccc@{}}
    \toprule
    Dataset & UT-scratch & UT-IM & IM-scratch & IM-IM \\
    \midrule
    \DTLforeach{ablations}{%
      \task=Column1,%
      \avgI=Column2,%
      \ciI=Column3,%
      \avgII=Column4,%
      \ciII=Column5,%
      \avgIII=Column6,%
      \ciIII=Column7,%
      \avgIX=Column8,%
      \ciIX=Column9%
    }{%
      \ifthenelse{\value{DTLrowi}=1}{}{%
        \ifthenelse{\value{DTLrowi}=9 \OR \value{DTLrowi}=14}{\\\midrule}{\\}%
      }%
      \dtlformat{\task}&%
      \dtlformat{\avgI} \ifthenelse{\value{DTLrowi}>13}{}{$\pm$ \dtlformat{\ciI}}\%&%
      \dtlformat{\avgII} \ifthenelse{\value{DTLrowi}>13}{}{$\pm$ \dtlformat{\ciII}}\%&%
      \dtlformat{\avgIII} \ifthenelse{\value{DTLrowi}>13}{}{$\pm$ \dtlformat{\ciIII}}\%&%
      \dtlformat{\avgIX} \ifthenelse{\value{DTLrowi}>13}{}{$\pm$ \dtlformat{\ciIX}}\%%
    }
    \\\bottomrule
  \end{tabular}
  \end{center}
  \end{table}
}

==> FLUTE (ICML 2021)/tables/ablations_wo_ci.tex <==
\begin{table}[h]
\ra{1.2}
\caption{\label{table:ablations_wo_ci} \emph{Left}: Exploring two alternative initialization schemes for each new task's $\Psi_h$ that don't rely on the Blender network: from scratch (`scratch') and from ImageNet's batch normalization parameters (`$\Psi_{IM}$'). \emph{Right}: Investigating the same two initialization schemes on a feature extractor that is trained on ImageNet only (instead of on all datasets as for FLUTE).}
\begin{center}
\scriptsize
\begin{tabular}{@{}lcc|cc@{}}
\toprule
\multicolumn{1}{l}{Training data} & \multicolumn{2}{c}{All (as in FLUTE)} & \multicolumn{2}{c}{ImageNet only} \\
$\Psi_h$ init scheme & scratch & $\Psi_{IM}$ & scratch & $\Psi_{IM}$ \\
\midrule
\DTLforeach{ablations}{%
  \task=Column1,%
  \avgI=Column2,%
  \ciI=Column3,%
  \avgII=Column4,%
  \ciII=Column5,%
  \avgIII=Column6,%
  \ciIII=Column7,%
  \avgIX=Column8,%
  \ciIX=Column9%
}{%
  \ifthenelse{\value{DTLrowi}=1}{}{%
    \ifthenelse{\value{DTLrowi}=9 \OR \value{DTLrowi}=14}{\\\midrule}{\\}%
  }%
  \dtlformat{\task}&%
  \dtlformat{\avgI} \ifthenelse{\value{DTLrowi}>13}{}{}\%&%
  \dtlformat{\avgII} \ifthenelse{\value{DTLrowi}>13}{}{}\%&%
  \dtlformat{\avgIII} \ifthenelse{\value{DTLrowi}>13}{}{}\%&%
  \dtlformat{\avgIX} \ifthenelse{\value{DTLrowi}>13}{}{}\%%
}
\\\bottomrule
\end{tabular}
\end{center}
\end{table}

==> FLUTE (ICML 2021)/tables/all.tex <==
\begin{table*}
\ra{1.2}
\caption{\label{table:main} Comparison of FLUTE to the previous state-of-the-art approaches on Meta-Dataset. The few-shot dataset generalization performance is shown in the last 5 rows (Traffic Signs - CIFAR-100), representing unseen datasets that require Strong Generalization (SG). For completeness, we also present results on the easier problem of Weak Generalization (WG) in the first 8 rows (ImageNet - Flower). We compare against CNAPs \cite{requeima2019fast}, TaskNorm \cite{bronskill2020tasknorm}, SimpleCNAPS \cite{bateni2019improved}, and the universal representation variants SUR(-pf) \cite{dvornik2020selecting} and URT(-pf) \cite{liu2020universal}. We emphasize that SUR and URT have 8 times more parameters compared to all other competitors (denoted by x8). FLUTE outperforms these previous methods by a significant margin for the problem of few-shot dataset generalization ($>5\%$ on Average SG) while still outperforming the state-of-the-art overall.}
\begin{center}
\scriptsize
\begin{tabular}{@{}lcccccccc@{}}
  \toprule
  Dataset & CNAPs & TaskNorm & SimpleCNAPs & SUR-pf & URT-pf & SUR (x8) & URT (x8) & FLUTE \\
  \midrule
  \DTLforeach{all}{%
    \task=Column1,%
    \avgI=Column2,%
    \ciI=Column3,%
    \avgII=Column4,%
    \ciII=Column5,%
    \avgIII=Column6,%
    \ciIII=Column7,%
    \avgIX=Column8,%
    \ciIX=Column9,%
    \avgX=Column10,%
    \ciX=Column11,%
    \avgXI=Column12,%
    \ciXI=Column13,%
    \avgXII=Column14,%
    \ciXII=Column15,%
    \avgXIII=Column16,%
    \ciXIII=Column17%
  }{%
    \ifthenelse{\value{DTLrowi}=1}{}{%
      \ifthenelse{\value{DTLrowi}=9 \OR \value{DTLrowi}=14}{\\\midrule}{\\}%
    }%
    \dtlformat{\task}&%
    \dtlformat{\avgI} \ifthenelse{\value{DTLrowi}>13}{}{$\pm$ \dtlformat{\ciI}}\%&%
    \dtlformat{\avgII} \ifthenelse{\value{DTLrowi}>13}{}{$\pm$ \dtlformat{\ciII}}\%&%
    \dtlformat{\avgIII} \ifthenelse{\value{DTLrowi}>13}{}{$\pm$ \dtlformat{\ciIII}}\%&%
    \dtlformat{\avgIX} \ifthenelse{\value{DTLrowi}>13}{}{$\pm$ \dtlformat{\ciIX}}\%&%
    \dtlformat{\avgX} \ifthenelse{\value{DTLrowi}>13}{}{$\pm$ \dtlformat{\ciX}}\%&%
    \dtlformat{\avgXI} \ifthenelse{\value{DTLrowi}>13}{}{$\pm$ \dtlformat{\ciXI}}\%&%
    \dtlformat{\avgXII} \ifthenelse{\value{DTLrowi}>13}{}{$\pm$ \dtlformat{\ciXII}}\%&%
    \dtlformat{\avgXIII} \ifthenelse{\value{DTLrowi}>13}{}{$\pm$ \dtlformat{\ciXIII}}\%%
  }
  \\\bottomrule
\end{tabular}
\end{center}
\end{table*}

==> FLUTE (ICML 2021)/tables/some.tex <==
{\onecolumn
  \begin{table}[ht]
  \ra{1.2}
  \caption{\label{table:all} All.}
  \begin{center}
  \scriptsize
  \begin{tabular}{@{}lcccccc@{}}
    \toprule
    Dataset & CNAPs & TaskNorm & SimpleCNAPs & SUR & URT & FLUTE \\
    \midrule
    \DTLforeach{all}{%
      \task=Column1,%
      \avgI=Column2,%
      \ciI=Column3,%
      \avgII=Column4,%
      \ciII=Column5,%
      \avgIII=Column6,%
      \ciIII=Column7,%
      \avgIX=Column8,%
      \ciIX=Column9,%
      \avgX=Column10,%
      \ciX=Column11,%
      \avgXI=Column12,%
      \ciXI=Column13%
    }{%
      \ifthenelse{\value{DTLrowi}=1}{}{%
        \ifthenelse{\value{DTLrowi}=9 \OR \value{DTLrowi}=14}{\\\midrule}{\\}%
      }%
      \dtlformat{\task}&%
      \dtlformat{\avgI} \ifthenelse{\value{DTLrowi}>13}{}{$\pm$ \dtlformat{\ciI}}\%&%
      \dtlformat{\avgII} \ifthenelse{\value{DTLrowi}>13}{}{$\pm$ \dtlformat{\ciII}}\%&%
      \dtlformat{\avgIII} \ifthenelse{\value{DTLrowi}>13}{}{$\pm$ \dtlformat{\ciIII}}\%&%
      \dtlformat{\avgIX} \ifthenelse{\value{DTLrowi}>13}{}{$\pm$ \dtlformat{\ciIX}}\%&%
      \dtlformat{\avgX} \ifthenelse{\value{DTLrowi}>13}{}{$\pm$ \dtlformat{\ciX}}\%&%
      \dtlformat{\avgXI} \ifthenelse{\value{DTLrowi}>13}{}{$\pm$ \dtlformat{\ciXI}}\%%
    }
    \\\bottomrule
  \end{tabular}
  \end{center}
  \end{table}
}

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}

==> source/acknowledgements.tex <==
\section*{Acknowledgements}

\red{TODO: WRITEME.}

==> source/experimental_setup.tex <==
\section{Experimental Setup}
% \red{TODO: WRITEME.}

% \red{Experiments to consider:}
% \begin{itemize}
%     \item \red{How does our approach perform when using SUR-pf parameters? Do we also bridge the unseen domain performance gap? If our hypothesis holds, then SUR-pf --- which was trained on ImageNet-only first and which only trained the domain-specific parameters afterwards for the other training domains --- should {\em not} benefit from the inductive bias of training a set of shared parameters that lend themselves well to multiple sets of domain-specific parameters.}
    
%     \item \red{Visualization of the (multi-level) dataset classifier's outputs for different test episodes coming from seen and unseen domains.}
    
%     \item \red{Table that compares PEGASUS against approaches with the same number of parameters (CNAPs, Simple CNAPs, Meta-Baseline, TaskNorm, SUR-pf, URT-pf).}
    
%     \item \red{Table that compares PEGASUS against the state-of-the-art models (SUR and URT) that contain significantly more parameters.}
% \end{itemize}
We conduct our experimental evaluation on the recent Meta-Dataset benchmark, which lends itself well to studying few-shot dataset generalization, as its designated training set is indeed comprised of diverse datasets, and its test set includes classes from previously-unseen datasets too.

\paragraph{Meta-Dataset} In more detail, the training set contains classes from ImageNet, Omniglot, Aircraft, Birds, Flowers, Quickdraw, Fungi, and Textures, some of which contain natural images (e.g. ImageNet, Birds, and Flowers), while others differ significantly in appearance. For example, Omniglot and Quickdraw depict hand drawings on a plain black background and Textures's images present perceptual characteristics of varying structure and don't feature a single object in the center of the image. The test set introduces two new datasets: Traffic Signs and MSCOCO, with the former differing significantly thematically from the training set (it depicts images of different traffic signs), and the latter, albeit thematically similar to ImageNet, has lower resolution and exhibits inclusion. Since the aim of this work is to study few-shot dataset generalization, we incorporate the 3 additional test datasets introduced in \citet{requeima2019fast}, to obtain a larger and more varied test set for this problem. These datasets are MNIST, CIFAR-10, and CIFAR-100.

\paragraph{Strong versus weak generalization} The problem of few-shot dataset generalization requires \emph{strong generalization} as there is a large generalization gap between the training and test distributions. Another popular, albeit easier, setting creates the test tasks from held-out classes of the datasets that were encountered at training time. This still falls within the umbrella of few-shot classification, as the test classes were not used for training, but is an easier problem since the generalization gap is inherently smaller. We thus refer to this setting as \emph{weak generalization}. %it is more likely that a feature extractor that works well on the training classes of a particular dataset may also work well on the test classes of the same dataset. From that point of view, this setup is closer to the traditional single-dataset few-shot classification problem and presents a \empy{weak generalization} problem. 
Although our focus is few-shot dataset generalization in this work, we also examine FLUTE's performance on the weak generalization tasks for completeness and compatibility with previous work.

We apply FLUTE in exactly the same way for this setting as described in Section~\ref{sec:flute}. In particular, despite the test classes originating from seen datasets in this setting, we are not told which of the $M$ datasets each task is sampled from. %\rz{I like this point about not knowing the dataaet at test time. This could be highlighted more}.
Therefore, we still require our Blender network to propose a blending of the $M$ sets of FiLM parameters as the initialization of $\Psi_{d^*}$, although we expect that it should almost exclusively select the correct dataset from which the task originates, assuming the dataset classifier is accurate.

\paragraph{Implementation details} Following the prior work, we use a ResNet-18 as the feature extractor. During training of our universal template, we treat each dataset-specific readout head $r_m$ as a cosine classifier (as in \citet{chen2019closer, chen2020new}): a linear layer without a bias, where both the layer inputs and the rows of the weight matrix are l2-normalized. We use stochastic gradient descent with momentum as the optimizer for this phase, with a cosine decay with restarts schedule for the learning rate. On the other hand, the second phase of training for our dataset classifier network converges quite quickly (around 14K steps). The design of the dataset classifier involves a deep set encoder, comprised by 5 convolutional layers, each followed by batch normalization and ReLU, with a standard linear readout on top. We use Adam for this phase. We report all details in the Appendix and we will open-source our code upon publication.

==> source/results.tex <==
\section{Results}

\begin{table*}
\ra{1.2}
\caption{\label{table:main} Comparison of FLUTE to the previous state-of-the-art approaches on Meta-Dataset. The few-shot dataset generalization performance is shown in the second group of rows (Traffic Signs - CIFAR-100), representing unseen datasets that require Strong Generalization (SG). For completeness, we also present results on the easier problem of Weak Generalization (WG) in the first 8 rows (ImageNet - Flower). We compare against CNAPs \cite{requeima2019fast}, TaskNorm \cite{bronskill2020tasknorm}, SimpleCNAPS \cite{bateni2019improved}, SUR(-pf) \cite{dvornik2020selecting} and URT(-pf) \cite{liu2020universal}. We emphasize that SUR and URT have 8 times more parameters compared to all other competitors (denoted by x8). FLUTE outperforms these previous methods by a significant margin for the problem of few-shot dataset generalization ($>5\%$ on Average SG) while still outperforming the state-of-the-art overall.}
\begin{center}
\scriptsize
\begin{tabular}{@{}lcccccccc@{}}
  \toprule
  Dataset & CNAPs & TaskNorm & SimpleCNAPs & SUR-pf & URT-pf & SUR (x8) & URT (x8) & FLUTE \\
  \midrule
  \DTLforeach{all}{%
    \task=Column1,%
    \avgI=Column2,%
    \ciI=Column3,%
    \avgII=Column4,%
    \ciII=Column5,%
    \avgIII=Column6,%
    \ciIII=Column7,%
    \avgIX=Column8,%
    \ciIX=Column9,%
    \avgX=Column10,%
    \ciX=Column11,%
    \avgXI=Column12,%
    \ciXI=Column13,%
    \avgXII=Column14,%
    \ciXII=Column15,%
    \avgXIII=Column16,%
    \ciXIII=Column17%
  }{%
    \ifthenelse{\value{DTLrowi}=1}{}{%
      \ifthenelse{\value{DTLrowi}=9 \OR \value{DTLrowi}=14}{\\\midrule}{\\}%
    }%
    \dtlformat{\task}&%
    \dtlformat{\avgI} \ifthenelse{\value{DTLrowi}>13}{}{$\pm$ \dtlformat{\ciI}}\%&%
    \dtlformat{\avgII} \ifthenelse{\value{DTLrowi}>13}{}{$\pm$ \dtlformat{\ciII}}\%&%
    \dtlformat{\avgIII} \ifthenelse{\value{DTLrowi}>13}{}{$\pm$ \dtlformat{\ciIII}}\%&%
    \dtlformat{\avgIX} \ifthenelse{\value{DTLrowi}>13}{}{$\pm$ \dtlformat{\ciIX}}\%&%
    \dtlformat{\avgX} \ifthenelse{\value{DTLrowi}>13}{}{$\pm$ \dtlformat{\ciX}}\%&%
    \dtlformat{\avgXI} \ifthenelse{\value{DTLrowi}>13}{}{$\pm$ \dtlformat{\ciXI}}\%&%
    \dtlformat{\avgXII} \ifthenelse{\value{DTLrowi}>13}{}{$\pm$ \dtlformat{\ciXII}}\%&%
    \dtlformat{\avgXIII} \ifthenelse{\value{DTLrowi}>13}{}{$\pm$ \dtlformat{\ciXIII}}\%%
  }
  \\\bottomrule
\end{tabular}
\end{center}
\end{table*}

\paragraph{Performance on Meta-Dataset} As our first experiment, we evaluate FLUTE on Meta-Dataset, in order to assess its performance on the challenging problem of few-shot dataset generalization, as well as on the weaker generalization setup. We compare against previous approaches that have the same number of parameters as FLUTE, as well as the state-of-the-art models on Meta-Dataset that use roughly 8 times more parameters than FLUTE. We present these results in Table~\ref{table:main}. We observe that FLUTE significantly outperforms all approaches on few-shot dataset generalization. Overall, it sets the new state-of-the-art on Meta-Dataset, despite FLUTE's compactness and parameter efficiency.
%\rz{This is the main result of the paper. It would be nice to figure out some way of bringing this out more. As it stands it is mentioned here and then you dive right into analysis and ablations.}\et{I totally agree. Let me know everyone if you have any suggestions on how to do this, I'm struggling to find a way to place more emphasis on this without taking up too much space.}

Having established FLUTE's effectiveness, we next take a closer look at the effect of its various design choices. %We also include additional analyses in the Appendix.
\begin{table}[h]
\ra{1.2}
\caption{\label{table:ablations_wo_ci} The effect of training on different data (`All', as in FLUTE, or `ImageNet-only'), and alternative initialization schemes for $\Psi_{d^*}$: from scratch (`scratch') and from ImageNet's FiLM parameters (`$\Psi_{IN}$'). The first column is the FLUTE model. We include confidence intervals for this table in the Appendix.}
\begin{center}
\scriptsize
\begin{tabular}{@{}l|c|cc|cc@{}}
\toprule
\multicolumn{1}{l}{Training data} & \multicolumn{1}{c}{All} & \multicolumn{2}{c}{All} & \multicolumn{2}{c}{ImageNet only} \\
\multicolumn{1}{l}{Init scheme} & Blender & Scratch & $\Psi_{IN}$ & Scratch & $\Psi_{IN}$\\
\midrule
\DTLforeach{ablations}{%
  \task=Column1,%
  \avgI=Column2,%
  \ciI=Column3,%
  \avgII=Column4,%
  \ciII=Column5,%
  \avgIII=Column6,%
  \ciIII=Column7,%
  \avgIX=Column8,%
  \ciIX=Column9,%
  \avgX=Column10,%
  \ciX=Column11,%
  \avgXI=Column12,%
  \ciXI=Column13%
}{%
  \ifthenelse{\value{DTLrowi}=1}{}{%
    \ifthenelse{\value{DTLrowi}=9 \OR \value{DTLrowi}=14}{\\\midrule}{\\}%
  }%
  \dtlformat{\task}&%
  \dtlformat{\avgI} \ifthenelse{\value{DTLrowi}>13}{}{}\%&%
%   \dtlformat{\avgXI} \ifthenelse{\value{DTLrowi}>13}{}{}\%&%
  \dtlformat{\avgII} \ifthenelse{\value{DTLrowi}>13}{}{}\%&%
  \dtlformat{\avgIII} \ifthenelse{\value{DTLrowi}>13}{}{}\%&%
  \dtlformat{\avgIX} \ifthenelse{\value{DTLrowi}>13}{}{}\%&%
  \dtlformat{\avgX} \ifthenelse{\value{DTLrowi}>13}{}{}\%%
%   \dtlformat{\avgXI} \ifthenelse{\value{DTLrowi}>13}{}{}\%%
}
\\\bottomrule
\end{tabular}
\end{center}
\end{table}

\paragraph{The importance of the Blender network} Recall that the role of this network is to propose an initialization for the FiLM parameters for each test task. We now explore two alternative ways of initializing those parameters: `from scratch' and `from ImageNet' ($\Psi_{IN}$). For each layer $i$, the former sets the additive terms $\beta_i$ to vectors of 0s, and the multiplicative terms $\gamma_i$ to vectors of 1s, while the latter sets the FiLM parameters throughout the network to those learned specifically for the ImageNet dataset, which we denote by $\Psi_{IN}$. We singled out ImageNet for this since it is often treated as a good source for transfer.

The results for this experiment are shown in the second and third  columns of Table~\ref{table:ablations_wo_ci} (the first shows FLUTE for reference). We find that initializing from $\Psi_{IN}$ yields impressive results on several datasets (e.g. ImageNet (unsurprisingly), but also Textures, CIFAR-10, CIFAR-100) but very poor results on datasets that are vastly different from ImageNet (e.g. Omiglot, Quickdraw, and Aircraft). On the other hand, initializing from scratch does not recover that strong performance on the ImageNet-like datasets, but evidently constitutes a much better solution for various other datasets (e.g. Omniglot, Quickraw and Aircraft). Therefore, the initialization of $\Psi_{d^*}$ really matters, with different techniques working best for different evaluation datasets. Our Blender network thus provides a good solution by tailoring the initialization to each task at hand, via the predicted compatibility with each training dataset.

\begin{figure*}[t]%
    \centering%
    \includegraphics[height=2.1cm]{figures/cifar10.pdf}%
    \includegraphics[height=2.1cm]{figures/cifar100.pdf}%
    \includegraphics[height=2.1cm]{figures/unshuffled_traffic_sign.pdf}%
    \includegraphics[height=2.1cm]{figures/mnist.pdf}%
    \includegraphics[height=2.1cm]{figures/mscoco.pdf}%
    \caption{The support and query accuracy over 600 test episodes of unseen datasets as a function of the fine-tuning steps for $\Psi_{d^*}$.}%
    \label{fig:fine_tuning}%
\end{figure*}

\paragraph{The importance of diverse training data}  Next, we empirically examine our hypothesis that training our feature extractor on \emph{all} training datasets is an important choice for encouraging (the convolutional layers of) our feature extractor to act as a universal template. In other words, had we not trained it on diverse data, perhaps it would be less general and thus less capable of supporting generalization to new datasets via merely changing the values of the batch normalization parameters. To investigate this, we trained a feature extractor (of identical architecture to FLUTE's) on ImageNet only. In this case, we only learn one set of FiLM parameters during training, since there is only one training dataset. We then attempt to tackle the test tasks similarly to FLUTE, by learning a new set of FiLM parameters for each, via one of the two initialization schemes proposed in the previous round of experiments.

The results produced by this ImageNet-only feature extractor are shown in the last two columns of Table~\ref{table:ablations_wo_ci}. We find that the feature extractor trained on all datasets performs significantly better across the board compared to that trained on ImageNet only, validating our hypothesis. Between the two initialization methods for the ImageNet-trained feature extractor, we still observe certain trade-offs like the ones identified for FLUTE's feature extractor, but notably, `from scratch' no longer performs well for datasets like Omniglot and Quickdraw as before. This speaks to the inferior generalizability of this feature extractor that was trained on less diverse data. Finally, we observe that even when evaluating on test classes from ImageNet (first row), FLUTE's feature extractor evidently constitutes a better template compared to the ImageNet-trained one, indicating positive transfer during FLUTE's multi-tasking training phase.

\begin{figure}%
    \centering%
    \includegraphics[width=\linewidth]{figures/heatmap.pdf}%
    \caption{\label{fig:heatmap} Visualization of the coefficients of the convex combination produced by the Blender network for various test datasets. Each column represents the average coefficients produced for 600 test tasks of a particular dataset.}%
\end{figure}

\paragraph{The effect of the number of steps to train $\Psi_{d^*}$} Figure~\ref{fig:fine_tuning} plots the support and query accuracy during the fine-tuning of the per-task parameters $\Psi_{d^*}$ on the support set, averaged over 600 test tasks of each unseen domain (strong generalization setting). We also show the corresponding plots for weak generalization in the Appendix. We used 6 steps for this, with a learning rate of 0.005, which are the values we used for FLUTE's results in Table~\ref{table:main}, chosen based on the validation set. We observe that some datasets benefit more than others from this fine-tuning. In fact, in some cases (CIFAR-100, MSCOCO) the support accuracy even decreases. This indicates that perhaps those hyperparameters aren't ideal for all test tasks. Moreover, the validation set may not be a good proxy for the test set, since it is comprised of different datasets, making hyperparameter selection hard. Tailoring the learning rate or number of steps to each task would be an interesting avenue for future work.  %Therefore, it is possible that a more aggressive learning rate would yield better results on episodes of held-out datasets. 
%We believe that discovering an appropriate model selection approach in this non-i.i.d. setting is an interesting direction for future work. 

\paragraph{Inspecting the Blender's proposals} We visualize the combination coefficients that the Blender produces for test tasks in Figure~\ref{fig:heatmap}. We notice that for test episodes of datasets seen during training (weak generalization setting), the Blender very strongly selects the dataset from which the task originated. For new datasets that did not appear in the training set (last 5 columns), the Blender seems to make reasonable choices (e.g. Quickdraw for MNIST, ImageNet for MSCOCO) but the probability distribution may be less peaky (e.g. for Traffic Signs and CIFAR-100). In the Appendix we also investigate the variance of these predictions across different test tasks within each dataset.
% \rz{Can we add a pointer to examining variance issue in Appendix?}

%\rz{One more general issue comes to mind here -- it is unclear what makes the method specific to dataset generalization. The UT parameters are initialized and adapted based on the support set in an episode. So they need not be consistent across episodes of a given dataset. The Blender is defined as a mixture across training datasets. Fig 2 shows the coefficients for test and train datasets. How much do these vary across episodes?}\et{Exactly, our method isn't specific to few-shot dataset generalization - it can also handle the weaker generalization problem of held-out classes of seen datasets. I was emphasizing dataset generalization throughout the paper in particular because that's the setting where we get the largest win compared to previous methods. :-) but let me know if you find this misleading? I find that the co-efficients are very consistent for seen datasets, and vary a bit more for unseen ones. Maybe we can add a visualization of the variance of these co-efficients for different datasets in the Appendix. What do you think?}.


\paragraph{Discussion} As alluded to earlier, an open challenge is defining an appropriate model selection mechanism for the difficult scenario when the provided validation set is not a good proxy for the test set. The problem that we study in this work, similarly to domain generalization \cite{gulrajani2020search},
%\rz{This paper has an extensive discussion of this issue} 
suffers from underspecification: there may be several solutions that all perform well on the training and validation sets but behave differently on the test set. With this in mind, perhaps we should adjust our evaluation metrics to account for this potential source of variance. For instance, in the context of FLUTE, we noticed in Table~\ref{table:ablations_wo_ci} that the initialization of $\Psi_{d^*}$ really matters, therefore perhaps the results are sensitive to the chosen checkpoint of the dataset classifier. We report in the Appendix the performance across more runs of that component and observe some variance on held-out datasets, but our conclusions hold across runs.

==> tables/ablations.tex <==
{\onecolumn
  \begin{table}[ht]
  \ra{1.2}
  \caption{\label{table:all} All.}
  \begin{center}
  \scriptsize
  \begin{tabular}{@{}lcccc@{}}
    \toprule
    Dataset & UT-scratch & UT-IM & IM-scratch & IM-IM \\
    \midrule
    \DTLforeach{ablations}{%
      \task=Column1,%
      \avgI=Column2,%
      \ciI=Column3,%
      \avgII=Column4,%
      \ciII=Column5,%
      \avgIII=Column6,%
      \ciIII=Column7,%
      \avgIX=Column8,%
      \ciIX=Column9%
    }{%
      \ifthenelse{\value{DTLrowi}=1}{}{%
        \ifthenelse{\value{DTLrowi}=9 \OR \value{DTLrowi}=14}{\\\midrule}{\\}%
      }%
      \dtlformat{\task}&%
      \dtlformat{\avgI} \ifthenelse{\value{DTLrowi}>13}{}{$\pm$ \dtlformat{\ciI}}\%&%
      \dtlformat{\avgII} \ifthenelse{\value{DTLrowi}>13}{}{$\pm$ \dtlformat{\ciII}}\%&%
      \dtlformat{\avgIII} \ifthenelse{\value{DTLrowi}>13}{}{$\pm$ \dtlformat{\ciIII}}\%&%
      \dtlformat{\avgIX} \ifthenelse{\value{DTLrowi}>13}{}{$\pm$ \dtlformat{\ciIX}}\%%
    }
    \\\bottomrule
  \end{tabular}
  \end{center}
  \end{table}
}

==> tables/ablations_wo_ci.tex <==
\begin{table}[h]
\ra{1.2}
\caption{\label{table:ablations_wo_ci} \emph{Left}: Exploring two alternative initialization schemes for each new task's $\Psi_h$ that don't rely on the Blender network: from scratch (`scratch') and from ImageNet's batch normalization parameters (`$\Psi_{IM}$'). \emph{Right}: Investigating the same two initialization schemes on a feature extractor that is trained on ImageNet only (instead of on all datasets as for FLUTE).}
\begin{center}
\scriptsize
\begin{tabular}{@{}lcc|cc@{}}
\toprule
\multicolumn{1}{l}{Training data} & \multicolumn{2}{c}{All (as in FLUTE)} & \multicolumn{2}{c}{ImageNet only} \\
$\Psi_h$ init scheme & scratch & $\Psi_{IM}$ & scratch & $\Psi_{IM}$ \\
\midrule
\DTLforeach{ablations}{%
  \task=Column1,%
  \avgI=Column2,%
  \ciI=Column3,%
  \avgII=Column4,%
  \ciII=Column5,%
  \avgIII=Column6,%
  \ciIII=Column7,%
  \avgIX=Column8,%
  \ciIX=Column9%
}{%
  \ifthenelse{\value{DTLrowi}=1}{}{%
    \ifthenelse{\value{DTLrowi}=9 \OR \value{DTLrowi}=14}{\\\midrule}{\\}%
  }%
  \dtlformat{\task}&%
  \dtlformat{\avgI} \ifthenelse{\value{DTLrowi}>13}{}{}\%&%
  \dtlformat{\avgII} \ifthenelse{\value{DTLrowi}>13}{}{}\%&%
  \dtlformat{\avgIII} \ifthenelse{\value{DTLrowi}>13}{}{}\%&%
  \dtlformat{\avgIX} \ifthenelse{\value{DTLrowi}>13}{}{}\%%
}
\\\bottomrule
\end{tabular}
\end{center}
\end{table}

==> tables/all.tex <==
\begin{table*}
\ra{1.2}
\caption{\label{table:main} Comparison of FLUTE to the previous state-of-the-art approaches on Meta-Dataset. The few-shot dataset generalization performance is shown in the last 5 rows (Traffic Signs - CIFAR-100), representing unseen datasets that require Strong Generalization (SG). For completeness, we also present results on the easier problem of Weak Generalization (WG) in the first 8 rows (ImageNet - Flower). We compare against CNAPs \cite{requeima2019fast}, TaskNorm \cite{bronskill2020tasknorm}, SimpleCNAPS \cite{bateni2019improved}, and the universal representation variants SUR(-pf) \cite{dvornik2020selecting} and URT(-pf) \cite{liu2020universal}. We emphasize that SUR and URT have 8 times more parameters compared to all other competitors (denoted by x8). FLUTE outperforms these previous methods by a significant margin for the problem of few-shot dataset generalization ($>5\%$ on Average SG) while still outperforming the state-of-the-art overall.}
\begin{center}
\scriptsize
\begin{tabular}{@{}lcccccccc@{}}
  \toprule
  Dataset & CNAPs & TaskNorm & SimpleCNAPs & SUR-pf & URT-pf & SUR (x8) & URT (x8) & FLUTE \\
  \midrule
  \DTLforeach{all}{%
    \task=Column1,%
    \avgI=Column2,%
    \ciI=Column3,%
    \avgII=Column4,%
    \ciII=Column5,%
    \avgIII=Column6,%
    \ciIII=Column7,%
    \avgIX=Column8,%
    \ciIX=Column9,%
    \avgX=Column10,%
    \ciX=Column11,%
    \avgXI=Column12,%
    \ciXI=Column13,%
    \avgXII=Column14,%
    \ciXII=Column15,%
    \avgXIII=Column16,%
    \ciXIII=Column17%
  }{%
    \ifthenelse{\value{DTLrowi}=1}{}{%
      \ifthenelse{\value{DTLrowi}=9 \OR \value{DTLrowi}=14}{\\\midrule}{\\}%
    }%
    \dtlformat{\task}&%
    \dtlformat{\avgI} \ifthenelse{\value{DTLrowi}>13}{}{$\pm$ \dtlformat{\ciI}}\%&%
    \dtlformat{\avgII} \ifthenelse{\value{DTLrowi}>13}{}{$\pm$ \dtlformat{\ciII}}\%&%
    \dtlformat{\avgIII} \ifthenelse{\value{DTLrowi}>13}{}{$\pm$ \dtlformat{\ciIII}}\%&%
    \dtlformat{\avgIX} \ifthenelse{\value{DTLrowi}>13}{}{$\pm$ \dtlformat{\ciIX}}\%&%
    \dtlformat{\avgX} \ifthenelse{\value{DTLrowi}>13}{}{$\pm$ \dtlformat{\ciX}}\%&%
    \dtlformat{\avgXI} \ifthenelse{\value{DTLrowi}>13}{}{$\pm$ \dtlformat{\ciXI}}\%&%
    \dtlformat{\avgXII} \ifthenelse{\value{DTLrowi}>13}{}{$\pm$ \dtlformat{\ciXII}}\%&%
    \dtlformat{\avgXIII} \ifthenelse{\value{DTLrowi}>13}{}{$\pm$ \dtlformat{\ciXIII}}\%%
  }
  \\\bottomrule
\end{tabular}
\end{center}
\end{table*}

==> tables/some.tex <==
{\onecolumn
  \begin{table}[ht]
  \ra{1.2}
  \caption{\label{table:all} All.}
  \begin{center}
  \scriptsize
  \begin{tabular}{@{}lcccccc@{}}
    \toprule
    Dataset & CNAPs & TaskNorm & SimpleCNAPs & SUR & URT & FLUTE \\
    \midrule
    \DTLforeach{all}{%
      \task=Column1,%
      \avgI=Column2,%
      \ciI=Column3,%
      \avgII=Column4,%
      \ciII=Column5,%
      \avgIII=Column6,%
      \ciIII=Column7,%
      \avgIX=Column8,%
      \ciIX=Column9,%
      \avgX=Column10,%
      \ciX=Column11,%
      \avgXI=Column12,%
      \ciXI=Column13%
    }{%
      \ifthenelse{\value{DTLrowi}=1}{}{%
        \ifthenelse{\value{DTLrowi}=9 \OR \value{DTLrowi}=14}{\\\midrule}{\\}%
      }%
      \dtlformat{\task}&%
      \dtlformat{\avgI} \ifthenelse{\value{DTLrowi}>13}{}{$\pm$ \dtlformat{\ciI}}\%&%
      \dtlformat{\avgII} \ifthenelse{\value{DTLrowi}>13}{}{$\pm$ \dtlformat{\ciII}}\%&%
      \dtlformat{\avgIII} \ifthenelse{\value{DTLrowi}>13}{}{$\pm$ \dtlformat{\ciIII}}\%&%
      \dtlformat{\avgIX} \ifthenelse{\value{DTLrowi}>13}{}{$\pm$ \dtlformat{\ciIX}}\%&%
      \dtlformat{\avgX} \ifthenelse{\value{DTLrowi}>13}{}{$\pm$ \dtlformat{\ciX}}\%&%
      \dtlformat{\avgXI} \ifthenelse{\value{DTLrowi}>13}{}{$\pm$ \dtlformat{\ciXI}}\%%
    }
    \\\bottomrule
  \end{tabular}
  \end{center}
  \end{table}
}
